The R-Process Alliance: Analysis of Limited-r Stars

Context. In recent years, the R-Process Alliance (RPA) has conducted a successful search for stars enhanced in elements produced by the rapid neutron-capture (r-)process. In particular, the RPA has uncovered a number of stars strongly enriched in light r-process elements, such as Sr, Y and Zr, the so-called limited-r stars, in order to investigate the astrophysical production site(s) of these elements. Aims. With this paper, we aim to investigate the possible formation sites for light neutron-capture elements, by deriving detailed abundances for neutron-capture elements from high-resolution, high signal-to-noise spectra of three limited-r stars. Methods. We conducted a 1D local thermodynamic equilibrium spectroscopic abundance analysis of three stars, as well as a kinematic analysis. Further, we calculated the lanthanide mass fraction (XLa) of our stars and of limited-r stars from the literature. Results. We found that the neutron-capture element abundance pattern of limited-r stars behaves differently depending on their [Ba/Eu]] ratios, and suggest that this should be taken into account in future investigations of their abundances. Furthermore, we found that the XLa of limited-r stars is lower than that of the kilonova AT2017gfo. The latter seems to be in the transition zone between limited-r XLa and that of r-I, r-II stars. Finally, we found that, unlike r-I and r-II stars, the current sample of limited-r stars are largely born in the Galaxy rather than being accreted.

==> Todo.tex <==
Goal to share with the rest of the RPA beginning of Nov and submit by Dec

Both:
Look at kinematic analysis of stars


Theodora:

Week 36
Merge Figures 1 and 2, add panels with Sr, Ba, and Eu, generally make more presentable; smaller labels, less white space between panels, maybe panels can share axis.

Week 37
Table 4+5 fix spaces, column alignment, remove .0 on N
Table 6 add references to caption, fix column alignment.

Discussion Section
Week 38
- Are these actually limited-r stars (for two yes, the third probably not)
- Match to baseline pattern, what does this imply and why do we do it. Add Figure.

Week 39
- Lanthanide fractions, what are the lanthanide fractions for the two limited r-stars, is that a better match to the 2017 kilonova (yes), but what are the limitations (solar r-patterns, viewing angle of kilonovae) 

Introduction to match discussion
Week 40
- site(s) of the r-process
Week 41
- lanthanide fraction and variations of this.
- Introduce the baseline pattern
Week 42
- the usefulness of limited-r stars and the RPA effort to find these 

Summary
Week 43
What did we do
Why did we do it
and what were the results


Terese
Week 36
Read/edit Observations section, add SNR to Table 1 (Done)
Week 37
Read/edit Stellar parameters and abundance analysis section (done)
Week 38 
Read/edit Result section (done)
Look at Li abundances - they look okay

Help with Discussion + introduction
- more details once Theodora has made a first draft.




==> abund_uncert_allstars.tex <==
\begin{table}
\caption{Uncertainties for the abundances of J003859+272551 due to the uncertainties in stellar parameteres.}
\centering
\begin{tabular}{cccccc}
\hline \hline
$\mathrm{Element}$ &  $\mathrm{\Delta T}_{eff}$ &  $\mathrm{\Delta \log}g$ &  $\mathrm{\Delta \xi}$ &  $\mathrm{\Delta [M/H]}$ &  $\mathrm{\sigma}_{sys}$ \\
& (dex) & (dex) &(dex) &(dex) & (dex)\\\hline\\
                 Li I &                         0.08 &                       -0.00 &                    0.01 &                      0.01 &                       0.07 \\
                 C-H &                         0.16 &                       -0.03 &                    0.01 &                      0.04 &                       0.10 \\
                 O I &                        -0.08 &                        0.04 &                   -0.01 &                     -0.00 &                       0.04 \\
                Na I &                         0.10 &                       -0.03 &                   -0.10 &                     -0.00 &                       0.16 \\
                Mg I &                         0.04 &                       -0.01 &                   -0.02 &                      0.00 &                       0.06 \\
                Al I &                         0.16 &                       -0.03 &                   -0.11 &                      0.01 &                       0.23 \\
                Si I &                         0.04 &                        0.01 &                   -0.02 &                     -0.00 &                       0.06 \\
                 K I &                         0.06 &                       -0.00 &                   -0.03 &                      0.00 &                       0.08 \\
                Ca I &                         0.04 &                        0.00 &                    0.01 &                      0.00 &                       0.04 \\
               Sc II &                         0.02 &                        0.03 &                   -0.01 &                      0.01 &                       0.06 \\
                Ti I &                         0.08 &                       -0.00 &                    0.03 &                      0.01 &                       0.05 \\
               Ti II &                         0.03 &                        0.03 &                    0.04 &                      0.02 &                       0.03 \\
                 V I &                         0.02 &                        0.01 &                    0.02 &                     -0.01 &                       0.02 \\
                V II &                        -0.02 &                        0.04 &                    0.01 &                      0.00 &                       0.01 \\
                Cr I &                         0.08 &                        0.00 &                    0.03 &                      0.01 &                       0.05 \\
               Cr II &                        -0.00 &                        0.03 &                   -0.01 &                      0.00 &                       0.03 \\
                Mn I &                         0.06 &                       -0.00 &                   -0.01 &                      0.00 &                       0.06 \\
                Fe I &                         0.04 &                        0.00 &                    0.03 &                      0.01 &                       0.02 \\
               Fe II &                         0.01 &                        0.03 &                    0.02 &                      0.01 &                       0.02 \\
                Co I &                         0.05 &                        0.01 &                   -0.02 &                     -0.01 &                       0.08 \\
                Ni I &                         0.04 &                        0.00 &                    0.03 &                      0.00 &                       0.02 \\
                Zn I &                         0.04 &                        0.01 &                   -0.01 &                      0.00 &                       0.06 \\
               Sr II &                        -0.10 &                       -0.04 &                   -0.19 &                     -0.10 &                       0.11 \\
                Y II &                        -0.00 &                        0.03 &                   -0.00 &                      0.01 &                       0.04 \\
               Zr II &                        -0.02 &                        0.04 &                    0.01 &                      0.00 &                       0.02 \\
               Ba II &                         0.03 &                        0.03 &                   -0.02 &                      0.01 &                       0.08 \\
               La II &                         0.02 &                        0.03 &                    0.03 &                      0.01 &                       0.02 \\
               Nd II &                         0.02 &                        0.02 &                    0.01 &                      0.02 &                       0.03 \\
               Eu II &                         0.02 &                        0.03 &                    0.02 &                      0.01 &                       0.03 \\
               Dy II &                         0.02 &                        0.03 &                    0.01 &                      0.03 &                       0.04 \\
               Er II &                         0.02 &                        0.03 &                   -0.07 &                     -0.01 &                       0.12 \\
               Yb II &                         0.06 &                        0.02 &                   -0.03 &                      0.01 &                       0.11 \\
               \hline
\end{tabular}
\tablefoot{}
\end{table}


\begin{table}
\caption{Uncertainties for the abundances of J20313531 due to the uncertainties in stellar parameteres.}
\centering
\begin{tabular}{cccccc}
\hline \hline
$\mathrm{Element}$ &  $\mathrm{\Delta T}_{eff}$ &  $\mathrm{\Delta \log}g$ &  $\mathrm{\Delta \xi}$ &  $\mathrm{\Delta [M/H]}$ &  $\mathrm{\sigma}_{sys}$ \\
& (dex) & (dex) &(dex) &(dex) & (dex)\\\hline\\
                Li I &                         0.06 &                       -0.01 &                   -0.00 &                      0.00 &                       0.04 \\
                C-H &                         0.11 &                       -0.04 &                    0.02 &                      0.05 &                       0.05  \\
                 O I &                        -0.07 &                        0.04 &                   -0.01 &                     -0.01 &                       0.02 \\
                Na I &                         0.04 &                       -0.01 &                   -0.04 &                     -0.00 &                       0.07 \\
                Mg I &                         0.06 &                       -0.03 &                   -0.03 &                      0.01 &                       0.06 \\
                Al I &                         0.14 &                       -0.00 &                   -0.01 &                      0.03 &                       0.14 \\
                Si I &                         0.02 &                       -0.00 &                   -0.00 &                      0.00 &                       0.02 \\
                 K I &                         0.05 &                       -0.01 &                   -0.04 &                     -0.00 &                       0.08 \\
                Ca I &                         0.04 &                       -0.00 &                    0.02 &                      0.00 &                       0.02 \\
               Sc II &                         0.01 &                        0.02 &                   -0.00 &                      0.01 &                       0.03 \\
                Ti I &                         0.07 &                       -0.00 &                    0.04 &                      0.01 &                       0.04 \\
               Ti II &                         0.02 &                        0.03 &                    0.04 &                      0.02 &                       0.02 \\
                 V I &                         0.02 &                        0.01 &                    0.01 &                     -0.01 &                       0.03 \\
                V II &                        -0.01 &                        0.02 &                    0.01 &                      0.01 &                       0.02 \\
                Cr I &                         0.07 &                       -0.00 &                    0.02 &                      0.01 &                       0.04 \\
               Cr II &                        -0.01 &                        0.03 &                   -0.01 &                      0.01 &                       0.03 \\
                Mn I &                         0.05 &                       -0.01 &                   -0.02 &                      0.00 &                       0.06 \\
               Mn II &                        -0.03 &                        0.01 &                   -0.06 &                     -0.00 &                       0.05 \\
                Fe I &                         0.04 &                       -0.00 &                    0.03 &                      0.01 &                       0.02 \\
               Fe II &                         0.00 &                        0.03 &                   -0.00 &                      0.01 &                       0.03 \\
                Co I &                         0.02 &                        0.00 &                   -0.01 &                     -0.01 &                       0.03 \\
                Ni I &                         0.04 &                        0.00 &                    0.03 &                      0.00 &                       0.02 \\
                Zn I &                         0.03 &                        0.01 &                   -0.01 &                      0.01 &                       0.05 \\
               Sr II &                         0.06 &                        0.01 &                   -0.09 &                      0.03 &                       0.15 \\
                Y II &                         0.01 &                        0.02 &                   -0.01 &                      0.02 &                       0.04 \\
               Zr II &                        -0.01 &                        0.04 &                    0.00 &                      0.00 &                       0.02 \\
               Ba II &                         0.02 &                        0.03 &                   -0.02 &                      0.02 &                       0.07 \\
               La II &                        -0.00 &                        0.03 &                    0.03 &                      0.02 &                       0.02 \\
               Nd II &                         0.02 &                        0.02 &                    0.02 &                      0.03 &                       0.03 \\
               Eu II &                         0.01 &                        0.03 &                    0.01 &                      0.02 &                       0.03 \\
               Dy II &                         0.01 &                        0.02 &                   -0.01 &                      0.02 &                       0.04 \\
               Er II &                         0.02 &                        0.02 &                   -0.02 &                      0.02 &                       0.06 \\
               Yb II &                         0.05 &                        0.03 &                   -0.03 &                      0.02 &                       0.10 \\
               \hline
\end{tabular}
\tablefoot{}
\end{table}


\begin{table}
\caption{Uncertainties for the abundances of J21402305 due to the uncertainties in stellar parameteres.}
\centering
\begin{tabular}{cccccc}
\hline \hline
$\mathrm{Element}$ &  $\mathrm{\Delta T}_{eff}$ &  $\mathrm{\Delta \log}g$ &  $\mathrm{\Delta \xi}$ &  $\mathrm{\Delta [M/H]}$ &  $\mathrm{\sigma}_{sys}$ \\
& (dex) & (dex) &(dex) &(dex) & (dex)\\\hline\\
                C-H &                         0.14 &                       -0.04 &                    0.04 &                      0.01 &                       0.07 \\
               N-H &                         0.16 &                       -0.08 &                   -0.05 &                     -0.02 &                       0.14 \\
                 O I &                        -0.07 &                        0.04 &                   -0.00 &                     -0.00 &                       0.04 \\
                Na I &                         0.13 &                       -0.09 &                   -0.08 &                     -0.02 &                       0.12 \\
                Mg I &                         0.04 &                       -0.01 &                   -0.02 &                      0.00 &                       0.04 \\
                Al I &                         0.25 &                       -0.09 &                   -0.09 &                     -0.01 &                       0.25 \\
                Si I &                         0.01 &                        0.00 &                   -0.01 &                     -0.02 &                       0.04 \\
                 K I &                         0.05 &                       -0.00 &                   -0.01 &                      0.00 &                       0.05 \\
                Ca I &                         0.04 &                       -0.00 &                    0.00 &                      0.00 &                       0.04 \\
               Sc II &                         0.02 &                        0.03 &                   -0.01 &                      0.00 &                       0.06 \\
                Ti I &                         0.07 &                       -0.00 &                    0.01 &                      0.00 &                       0.06 \\
               Ti II &                         0.04 &                        0.05 &                    0.06 &                      0.01 &                       0.04 \\
                 V I &                         0.02 &                        0.00 &                    0.02 &                     -0.01 &                       0.02 \\
                V II &                         0.00 &                        0.04 &                    0.00 &                      0.00 &                       0.04 \\
                Cr I &                         0.07 &                       -0.00 &                    0.03 &                      0.01 &                       0.05 \\
               Cr II &                         0.00 &                        0.04 &                   -0.01 &                      0.00 &                       0.05 \\
                Mn I &                         0.04 &                       -0.02 &                   -0.02 &                     -0.00 &                       0.04 \\
               Mn II &                        -0.01 &                        0.02 &                   -0.04 &                      0.01 &                       0.05 \\
                Fe I &                         0.05 &                        0.00 &                    0.04 &                      0.01 &                       0.03 \\
               Fe II &                         0.02 &                        0.04 &                    0.01 &                      0.01 &                       0.05 \\
                Co I &                         0.04 &                       -0.00 &                   -0.02 &                     -0.01 &                       0.05 \\
                Ni I &                         0.04 &                        0.00 &                    0.04 &                      0.00 &                       0.02 \\
                Cu I &                         0.04 &                        0.00 &                    0.01 &                      0.01 &                       0.03 \\
                Zn I &                         0.04 &                        0.01 &                   -0.02 &                      0.00 &                       0.07 \\
                Sr I &                         0.04 &                       -0.01 &                   -0.00 &                      0.00 &                       0.04 \\
               Sr II &                        -0.00 &                        0.03 &                   -0.01 &                      0.00 &                       0.03 \\
                Y II &                        -0.03 &                        0.03 &                   -0.01 &                      0.01 &                       0.02 \\
               Zr II &                         0.01 &                        0.05 &                    0.02 &                      0.01 &                       0.04 \\
               Ba II &                         0.05 &                        0.03 &                   -0.03 &                      0.00 &                       0.10 \\
               La II &                         0.24 &                        0.05 &                    0.01 &                      0.05 &                       0.26 \\
               Nd II &                         0.04 &                        0.04 &                    0.02 &                      0.01 &                       0.06 \\
               Eu II &                        -0.01 &                        0.06 &                    0.03 &                      0.01 &                       0.03 \\
               Er II &                         0.05 &                        0.05 &                   -0.15 &                     -0.01 &                       0.24 \\
               Yb II &                         0.09 &                        0.04 &                   -0.05 &                      0.01 &                       0.17 
               \\\hline
\end{tabular}
\tablefoot{}
\end{table}

==> line_info_table_final.tex <==
\begin{table}
\caption{Sample of line info.}
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ccccccccc}
\hline \hline
$\mathrm{Stellar ID}$ &  $\mathrm{Species}$ &  $\mathrm{\lambda}$ &  $\mathrm{\chi}$ &  $\mathrm{\log\,}gf$ &  $\mathrm{EW}$& $\sigma_{\mathrm{EW}}$ &$\mathrm{\log \epsilon}$ & $\mathrm{ref}$\\
&  & ($\AA$) &($\mathrm{eV}$) & & ($\mathrm{m}\AA$)& ($\mathrm{m}\AA$)&&\\ \hline
J003859  &      O I  & 7771.94 &    9.15  &    0.37  & 20.48 & 2.62 & 7.65 & 1 \\
   J003859  &      O I  & 7774.17 &    9.15  &    0.22  & 7.73 & 1.62 & 7.24 & 1 \\
   J003859  &      O I  & 7775.39 &    9.15  &    0.00  & 7.87 & 1.53 & 7.47 & 1 \\
   J003859  &     Na I  & 5889.95 &    0.00  &    0.11  & 170.38 & 2.93 & 4.21 & 1 \\
   J003859  &     Na I  & 5895.92 &    0.00  &   -0.19  & 158.03 & 0.78 & 4.36 & 1 \\
   J003859  &     Mg I  & 4167.27 &    4.35  &   -0.74  & 61.95 & 1.21 & 5.66 & 1 \\
   J003859  &     Mg I  & 4702.99 &    4.33  &   -0.44  & 80.18 & 0.71 & 5.54 & 1 \\
   J003859  &     Mg I  & 5528.40 &    4.35  &   -0.55  & 79.94 & 0.71 & 5.68 & 2 \\
   J003859  &     Mg I  & 5711.09 &    4.35  &   -1.84  & 14.72 & 0.80 & 5.79 & 2 \\
   J003859  &     Al I  & 3961.52 &    0.01  &   -0.33  & 121.84 & 1.40 & 3.35 & 1 \\
   J003859  &     Si I  & 5772.15 &    5.08  &   -1.75  & 5.58 & 1.21 & 5.98 & 1 \\
   J003859  &      K I  & 7664.90 &    0.00  &    0.12  & 65.09 & 0.89 & 3.37 & 1 \\
   J003859  &      K I  & 7698.96 &    0.00  &   -0.18  & 45.82 & 0.88 & 3.33 & 1 \\
   J003859  &     Ca I  & 4318.65 &    1.90  &   -0.21  & 54.54 & 0.86 & 4.16 & 1 \\
   J003859  &     Ca I  & 4425.44 &    1.88  &   -0.41  & 56.26 & 0.76 & 4.35 & 3 \\
   J003859  &     Ca I  & 4435.69 &    1.89  &   -0.55  & 48.98 & 0.71 & 4.37 & 3 \\
   J003859  &     Ca I  & 4454.78 &    1.90  &    0.26  & 82.91 & 0.81 & 4.20 & 1 \\
   J003859  &     Ca I  & 4455.89 &    1.90  &   -0.55  & 43.90 & 0.79 & 4.29 & 3 \\
   J003859  &     Ca I  & 4526.94 &    2.71  &   -0.47  & 9.86 & 0.72 & 4.20 & 3 \\
   J003859  &     Ca I  & 4578.55 &    2.52  &   -0.67  & 12.93 & 0.86 & 4.33 & 3 \\
   J003859  &     Ca I  & 5261.71 &    2.52  &   -0.60  & 16.33 & 1.00 & 4.35 & 3 \\
   J003859  &     Ca I  & 5581.97 &    2.52  &   -0.58  & 13.93 & 0.70 & 4.24 & 3 \\
   J003859  &     Ca I  & 5588.76 &    2.52  &    0.30  & 52.36 & 0.69 & 4.21 & 3 \\
   J003859  &     Ca I  & 5590.12 &    2.52  &   -0.60  & 14.81 & 0.71 & 4.29 & 3 \\
   J003859  &     Ca I  & 5601.29 &    2.53  &   -0.57  & 17.23 & 0.55 & 4.35 & 3 \\
   J003859  &     Ca I  & 5857.45 &    2.93  &    0.17  & 32.41 & 0.64 & 4.40 & 3 \\
   J003859  &     Ca I  & 6102.72 &    1.88  &   -0.81  & 41.10 & 0.50 & 4.40 & 3 \\
   J003859  &     Ca I  & 6122.22 &    1.89  &   -0.33  & 66.27 & 0.66 & 4.37 & 3 \\
   J003859  &     Ca I  & 6161.29 &    2.52  &   -1.35  & 6.38 & 0.93 & 4.62 & 3 \\
   J003859  &     Ca I  & 6162.17 &    1.90  &   -0.11  & 81.07 & 0.61 & 4.42 & 3 \\
   J003859  &     Ca I  & 6166.44 &    2.52  &   -1.22  & 5.91 & 0.59 & 4.45 & 3 \\
   J003859  &     Ca I  & 6169.06 &    2.52  &   -0.87  & 12.77 & 0.65 & 4.47 & 3 \\
   J003859  &     Ca I  & 6169.56 &    2.53  &   -0.60  & 21.99 & 0.66 & 4.50 & 3 \\
   J003859  &     Ca I  & 6449.81 &    2.52  &   -0.55  & 20.10 & 0.83 & 4.38 & 3 \\
   J003859  &     Ca I  & 6471.66 &    2.53  &   -0.71  & 18.17 & 0.86 & 4.50 & 3 \\
   J003859  &     Ca I  & 6499.65 &    2.52  &   -0.81  & 15.70 & 0.77 & 4.51 & 3 \\
   J003859  &     Ca I  & 6717.69 &    2.71  &   -0.58  & 17.04 & 0.82 & 4.51 & 3 \\
   J003859  &     Ti I  & 3989.76 &    0.02  &   -0.13  & 69.26 & 1.38 & 3.01 & 4 \\
   J003859  &     Ti I  & 3998.64 &    0.05  &    0.02  & 63.54 & 1.02 & 2.76 & 4 \\
   J003859  &     Ti I  & 4512.73 &    0.84  &   -0.40  & 14.45 & 1.12 & 2.94 & 4 \\
   J003859  &     Ti I  & 4518.02 &    0.83  &   -0.25  & 16.76 & 1.42 & 2.85 & 4 \\
   J003859  &     Ti I  & 4533.24 &    0.85  &    0.54  & 49.93 & 0.69 & 2.79 & 4 \\
   J003859  &     Ti I  & 4534.78 &    0.84  &    0.35  & 42.64 & 0.67 & 2.83 & 4 \\
   J003859  &     Ti I  & 4548.76 &    0.83  &   -0.28  & 17.85 & 0.81 & 2.91 & 4 \\
   J003859  &     Ti I  & 4555.48 &    0.85  &   -0.40  & 11.73 & 0.68 & 2.84 & 4 \\
   J003859  &     Ti I  & 4681.91 &    0.05  &   -1.01  & 25.09 & 0.68 & 2.97 & 1 \\
   J003859  &     Ti I  & 4840.87 &    0.90  &   -0.43  & 12.27 & 0.74 & 2.93 & 4 \\
   J003859  &     Ti I  & 4981.73 &    0.84  &    0.57  & 56.79 & 0.71 & 2.83 & 4 \\
   J003859  &     Ti I  & 4999.50 &    0.83  &    0.32  & 42.42 & 0.64 & 2.81 & 4 \\
   J003859  &     Ti I  & 5064.65 &    0.05  &   -0.94  & 28.37 & 0.77 & 2.94 & 4 \\
   J003859  &     Ti I  & 5173.74 &    0.00  &   -1.06  & 21.44 & 0.71 & 2.84 & 4 \\
   J003859  &     Ti I  & 5192.97 &    0.02  &   -0.95  & 31.49 & 0.86 & 2.97 & 4 \\
   J003859  &     Ti I  & 5210.38 &    0.05  &   -0.82  & 37.41 & 0.69 & 2.99 & 4 \\
   J003859  &    Ti II  & 3761.32 &    0.57  &    0.18  & 161.05 & 2.10 & 3.01 & 5 \\
   J003859  &    Ti II  & 4028.34 &    1.89  &   -0.92  & 49.35 & 0.97 & 2.87 & 5 \\
   J003859  &    Ti II  & 4337.91 &    1.08  &   -0.96  & 84.92 & 0.79 & 2.73 & 6 \\
   J003859  &    Ti II  & 4394.06 &    1.22  &   -1.77  & 46.90 & 0.85 & 2.89 & 5 \\
   J003859  &    Ti II  & 4395.84 &    1.24  &   -1.93  & 34.91 & 0.87 & 2.85 & 5 \\
   J003859  &    Ti II  & 4399.77 &    1.24  &   -1.20  & 83.05 & 0.83 & 3.08 & 5 \\
   J003859  &    Ti II  & 4409.52 &    1.23  &   -2.53  & 14.45 & 0.76 & 2.94 & 5 \\
   J003859  &    Ti II  & 4417.71 &    1.17  &   -1.19  & 78.08 & 0.69 & 2.87 & 6 \\
   J003859  &    Ti II  & 4418.33 &    1.24  &   -1.99  & 38.86 & 0.70 & 2.99 & 5 \\
   J003859  &    Ti II  & 4443.80 &    1.08  &   -0.71  & 102.89 & 0.65 & 2.91 & 5 \\
   J003859  &    Ti II  & 4444.55 &    1.12  &   -2.20  & 35.79 & 0.76 & 3.00 & 5 \\
   J003859  &    Ti II  & 4450.48 &    1.08  &   -1.52  & 73.43 & 0.90 & 3.00 & 5 \\
   J003859  &    Ti II  & 4464.45 &    1.16  &   -1.81  & 54.32 & 0.71 & 2.99 & 6 \\
   J003859  &    Ti II  & 4470.85 &    1.17  &   -2.02  & 27.24 & 0.97 & 2.70 & 6 \\
   J003859  &    Ti II  & 4493.52 &    1.08  &   -2.78  & 12.73 & 0.89 & 2.95 & 5 \\
   J003859  &    Ti II  & 4501.27 &    1.12  &   -0.77  & 104.33 & 0.67 & 3.04 & 5 \\
   J003859  &    Ti II  & 4571.97 &    1.57  &   -0.31  & 98.23 & 0.79 & 2.90 & 5 \\
   J003859  &    Ti II  & 4583.41 &    1.16  &   -2.84  & 12.58 & 0.75 & 3.09 & 5 \\
   J003859  &    Ti II  & 4708.66 &    1.24  &   -2.35  & 22.86 & 0.66 & 2.99 & 5 \\
   J003859  &    Ti II  & 4798.53 &    1.08  &   -2.66  & 20.84 & 1.06 & 3.06 & 5 \\
   J003859  &    Ti II  & 5129.16 &    1.89  &   -1.34  & 34.58 & 1.67 & 2.92 & 5 \\
   J003859  &    Ti II  & 5185.90 &    1.89  &   -1.41  & 31.57 & 0.94 & 2.92 & 5 \\
   J003859  &    Ti II  & 5336.79 &    1.58  &   -1.60  & 37.93 & 0.64 & 2.88 & 5 \\
   J003859  &    Ti II  & 5381.02 &    1.57  &   -1.97  & 25.62 & 0.60 & 2.99 & 5 \\
   J003859  &    Ti II  & 5418.77 &    1.58  &   -2.13  & 18.93 & 1.37 & 3.00 & 5 \\
   J003859  &     Cr I  & 4289.72 &    0.00  &   -0.37  & 97.28 & 0.87 & 3.08 & 7 \\
   J003859  &     Cr I  & 4545.95 &    0.94  &   -1.37  & 13.08 & 0.71 & 3.15 & 7 \\
   J003859  &     Cr I  & 5206.04 &    0.94  &    0.02  & 70.56 & 0.63 & 2.94 & 7 \\
   J003859  &     Cr I  & 5296.69 &    0.98  &   -1.36  & 14.89 & 0.70 & 3.20 & 7 \\
   J003859  &     Cr I  & 5298.28 &    0.98  &   -1.14  & 20.24 & 1.16 & 3.14 & 7 \\
   J003859  &     Cr I  & 5345.80 &    1.00  &   -0.95  & 26.06 & 0.83 & 3.11 & 7 \\
   J003859  &     Cr I  & 5348.31 &    1.00  &   -1.21  & 22.32 & 2.05 & 3.28 & 7 \\
   J003859  &     Cr I  & 5409.77 &    1.03  &   -0.67  & 39.16 & 0.73 & 3.13 & 7 \\
   J003859  &    Cr II  & 4558.64 &    4.07  &   -0.43  & 18.51 & 0.74 & 3.13 & 8 \\
   J003859  &    Cr II  & 4588.20 &    4.07  &   -0.65  & 14.39 & 0.67 & 3.22 & 8 \\
   J003859  &    Cr II  & 4592.05 &    4.07  &   -1.30  & 4.78 & 0.71 & 3.34 & 8 \\
   J003859  &     Fe I  & 3742.62 &    2.94  &   -0.81  & 45.13 & 2.13 & 5.16 & 9 \\
   J003859  &     Fe I  & 3765.54 &    3.24  &    0.48  & 74.36 & 2.04 & 4.85 & 10 \\
   J003859  &     Fe I  & 3786.68 &    1.01  &   -2.18  & 74.27 & 1.50 & 5.10 & 10 \\
   J003859  &     Fe I  & 3805.34 &    3.30  &    0.31  & 60.56 & 1.45 & 4.75 & 10 \\
   J003859  &     Fe I  & 3808.73 &    2.56  &   -1.17  & 44.42 & 1.50 & 5.10 & 11 \\
   J003859  &     Fe I  & 3902.95 &    1.56  &   -0.44  & 116.31 & 1.26 & 4.97 & 10 \\
   J003859  &     Fe I  & 3920.26 &    0.12  &   -1.73  & 124.77 & 1.08 & 5.00 & 10 \\
   J003859  &     Fe I  & 3949.95 &    2.18  &   -1.25  & 57.94 & 1.11 & 5.02 & 10 \\
   J003859  &     Fe I  & 3977.74 &    2.20  &   -1.12  & 63.01 & 1.08 & 5.02 & 10 \\
   J003859  &     Fe I  & 4067.98 &    3.21  &   -0.53  & 45.33 & 1.00 & 5.13 & 9 \\
   J003859  &     Fe I  & 4070.77 &    3.24  &   -0.87  & 24.96 & 1.38 & 5.08 & 9 \\
   J003859  &     Fe I  & 4114.44 &    2.83  &   -1.30  & 26.52 & 0.92 & 5.11 & 10 \\
   J003859  &     Fe I  & 4132.06 &    1.61  &   -0.68  & 116.95 & 1.05 & 5.21 & 10 \\
   J003859  &     Fe I  & 4134.68 &    2.83  &   -0.65  & 54.52 & 0.97 & 5.02 & 10 \\
   J003859  &     Fe I  & 4143.87 &    1.56  &   -0.51  & 116.42 & 0.88 & 4.98 & 10 \\
   J003859  &     Fe I  & 4147.67 &    1.49  &   -2.07  & 71.79 & 0.90 & 5.36 & 10 \\
   J003859  &     Fe I  & 4150.25 &    3.43  &   -1.19  & 13.34 & 1.03 & 5.26 & 9 \\
   J003859  &     Fe I  & 4157.78 &    3.42  &   -0.40  & 37.30 & 0.92 & 5.07 & 10 \\
   J003859  &     Fe I  & 4158.79 &    3.43  &   -0.70  & 20.18 & 0.90 & 4.99 & 9 \\
   J003859  &     Fe I  & 4175.64 &    2.85  &   -0.83  & 50.22 & 0.82 & 5.14 & 10 \\
   J003859  &     Fe I  & 4182.38 &    3.02  &   -1.18  & 23.13 & 1.13 & 5.11 & 10 \\
   J003859  &     Fe I  & 4184.89 &    2.83  &   -0.87  & 47.33 & 0.90 & 5.10 & 10 \\
   J003859  &     Fe I  & 4187.04 &    2.45  &   -0.56  & 77.69 & 0.95 & 4.99 & 12 \\
   J003859  &     Fe I  & 4187.80 &    2.42  &   -0.51  & 83.76 & 1.08 & 5.05 & 10 \\
   J003859  &     Fe I  & 4191.43 &    2.47  &   -0.67  & 68.78 & 0.83 & 4.92 & 10 \\
   J003859  &     Fe I  & 4195.33 &    3.33  &   -0.49  & 49.69 & 1.15 & 5.30 & 10 \\
   J003859  &     Fe I  & 4199.10 &    3.05  &    0.16  & 74.54 & 0.84 & 4.89 & 10 \\
   J003859  &     Fe I  & 4202.03 &    1.49  &   -0.69  & 105.64 & 0.82 & 4.83 & 10 \\
   J003859  &     Fe I  & 4216.18 &    0.00  &   -3.36  & 87.87 & 0.80 & 5.41 & 10 \\
   J003859  &     Fe I  & 4217.55 &    3.43  &   -0.48  & 32.06 & 0.81 & 5.04 & 10 \\
   J003859  &     Fe I  & 4222.21 &    2.45  &   -0.91  & 63.08 & 0.79 & 5.02 & 10 \\
   J003859  &     Fe I  & 4227.43 &    3.33  &    0.27  & 80.68 & 1.03 & 5.22 & 10 \\
   J003859  &     Fe I  & 4233.60 &    2.48  &   -0.60  & 76.06 & 0.91 & 5.02 & 12 \\
   J003859  &     Fe I  & 4238.81 &    3.40  &   -0.23  & 45.40 & 0.88 & 5.02 & 10 \\
   J003859  &     Fe I  & 4250.12 &    2.47  &   -0.38  & 87.99 & 0.88 & 5.05 & 10 \\
   J003859  &     Fe I  & 4250.79 &    1.56  &   -0.71  & 108.94 & 0.76 & 4.99 & 10 \\
   J003859  &     Fe I  & 4260.47 &    2.40  &    0.08  & 103.71 & 0.82 & 4.86 & 10 \\
   J003859  &     Fe I  & 4282.40 &    2.18  &   -0.78  & 74.22 & 0.74 & 4.87 & 10 \\
   J003859  &     Fe I  & 4415.12 &    1.61  &   -0.62  & 118.58 & 0.72 & 5.11 & 10 \\
   J003859  &     Fe I  & 4430.61 &    2.22  &   -1.73  & 42.01 & 0.75 & 5.17 & 10 \\
   J003859  &     Fe I  & 4442.34 &    2.20  &   -1.23  & 73.13 & 0.72 & 5.25 & 10 \\
   J003859  &     Fe I  & 4447.72 &    2.22  &   -1.36  & 59.58 & 0.69 & 5.12 & 11 \\
   J003859  &     Fe I  & 4461.65 &    0.09  &   -3.19  & 89.59 & 0.67 & 5.33 & 10 \\
   J003859  &     Fe I  & 4466.55 &    2.83  &   -0.60  & 68.30 & 0.69 & 5.23 & 10 \\
   J003859  &     Fe I  & 4484.22 &    3.60  &   -0.64  & 21.01 & 4.61 & 5.11 & 9 \\
   J003859  &     Fe I  & 4489.74 &    0.12  &   -3.90  & 58.61 & 0.76 & 5.34 & 10 \\
   J003859  &     Fe I  & 4494.56 &    2.20  &   -1.14  & 69.95 & 0.66 & 5.09 & 10 \\
   J003859  &     Fe I  & 4531.15 &    1.48  &   -2.10  & 65.01 & 0.69 & 5.16 & 10 \\
   J003859  &     Fe I  & 4547.85 &    3.55  &   -0.82  & 14.87 & 0.78 & 5.05 & 11 \\
   J003859  &     Fe I  & 4592.65 &    1.56  &   -2.46  & 49.55 & 0.70 & 5.30 & 10 \\
   J003859  &     Fe I  & 4602.00 &    1.61  &   -3.13  & 14.50 & 0.72 & 5.25 & 10 \\
   J003859  &     Fe I  & 4602.94 &    1.49  &   -2.21  & 63.68 & 0.69 & 5.25 & 10 \\
   J003859  &     Fe I  & 4619.29 &    3.60  &   -1.06  & 10.66 & 0.77 & 5.17 & 9 \\
   J003859  &     Fe I  & 4630.12 &    2.28  &   -2.58  & 12.22 & 0.88 & 5.34 & 11 \\
   J003859  &     Fe I  & 4733.59 &    1.49  &   -2.99  & 24.90 & 0.72 & 5.26 & 10 \\
   J003859  &     Fe I  & 4736.77 &    3.21  &   -0.67  & 39.94 & 0.71 & 5.12 & 9 \\
   J003859  &     Fe I  & 4786.81 &    3.02  &   -1.61  & 10.90 & 0.66 & 5.10 & 10 \\
   J003859  &     Fe I  & 4789.65 &    3.55  &   -0.96  & 14.44 & 0.80 & 5.16 & 10 \\
   J003859  &     Fe I  & 4871.32 &    2.87  &   -0.34  & 71.30 & 0.73 & 5.00 & 12 \\
   J003859  &     Fe I  & 4872.14 &    2.88  &   -0.57  & 60.88 & 0.76 & 5.04 & 10 \\
   J003859  &     Fe I  & 4890.76 &    2.88  &   -0.38  & 71.76 & 0.89 & 5.06 & 12 \\
   J003859  &     Fe I  & 4891.49 &    2.85  &   -0.11  & 82.20 & 0.87 & 4.97 & 10 \\
   J003859  &     Fe I  & 4903.31 &    2.88  &   -0.89  & 45.02 & 0.72 & 5.06 & 12 \\
   J003859  &     Fe I  & 4910.02 &    3.40  &   -1.28  & 9.18 & 0.77 & 5.09 & 9 \\
   J003859  &     Fe I  & 4918.99 &    2.86  &   -0.34  & 71.56 & 0.66 & 4.99 & 10 \\
   J003859  &     Fe I  & 4920.50 &    2.83  &    0.07  & 91.89 & 0.69 & 4.97 & 10 \\
   J003859  &     Fe I  & 4924.77 &    2.28  &   -2.11  & 20.68 & 0.69 & 5.12 & 10 \\
   J003859  &     Fe I  & 4938.81 &    2.88  &   -1.08  & 37.82 & 0.73 & 5.12 & 10 \\
   J003859  &     Fe I  & 4939.69 &    0.86  &   -3.25  & 49.53 & 0.73 & 5.29 & 10 \\
   J003859  &     Fe I  & 4946.39 &    3.37  &   -1.11  & 24.25 & 16.30 & 5.39 & 12 \\
   J003859  &     Fe I  & 4966.09 &    3.33  &   -0.79  & 27.60 & 0.88 & 5.10 & 9 \\
   J003859  &     Fe I  & 4994.13 &    0.92  &   -2.97  & 59.15 & 0.62 & 5.25 & 10 \\
   J003859  &     Fe I  & 5001.86 &    3.88  &   -0.01  & 31.02 & 0.73 & 4.99 & 12 \\
   J003859  &     Fe I  & 5005.71 &    3.88  &   -0.12  & 25.95 & 0.70 & 4.99 & 12 \\
   J003859  &     Fe I  & 5006.12 &    2.83  &   -0.62  & 60.74 & 0.66 & 5.02 & 10 \\
   J003859  &     Fe I  & 5014.94 &    3.94  &   -0.18  & 22.73 & 0.81 & 5.03 & 9 \\
   J003859  &     Fe I  & 5022.24 &    3.98  &   -0.33  & 13.27 & 0.89 & 4.93 & 12 \\
   J003859  &     Fe I  & 5044.21 &    2.85  &   -2.02  & 11.04 & 0.93 & 5.32 & 10 \\
   J003859  &     Fe I  & 5049.82 &    2.28  &   -1.36  & 59.86 & 0.73 & 5.15 & 10 \\
   J003859  &     Fe I  & 5051.63 &    0.92  &   -2.76  & 70.78 & 0.67 & 5.27 & 10 \\
   J003859  &     Fe I  & 5068.77 &    2.94  &   -1.04  & 34.92 & 0.70 & 5.08 & 10 \\
   J003859  &     Fe I  & 5079.74 &    0.99  &   -3.24  & 43.21 & 0.65 & 5.30 & 10 \\
   J003859  &     Fe I  & 5083.34 &    0.96  &   -2.84  & 57.36 & 0.65 & 5.13 & 10 \\
   J003859  &     Fe I  & 5123.72 &    1.01  &   -3.06  & 55.16 & 0.70 & 5.36 & 10 \\
   J003859  &     Fe I  & 5127.36 &    0.92  &   -3.25  & 45.17 & 0.70 & 5.26 & 10 \\
   J003859  &     Fe I  & 5131.47 &    2.22  &   -2.52  & 16.53 & 0.84 & 5.33 & 10 \\
   J003859  &     Fe I  & 5133.69 &    4.18  &    0.36  & 32.46 & 0.68 & 4.96 & 9 \\
   J003859  &     Fe I  & 5141.74 &    2.42  &   -2.24  & 16.92 & 0.76 & 5.28 & 10 \\
   J003859  &     Fe I  & 5150.84 &    0.99  &   -3.04  & 48.38 & 0.68 & 5.19 & 10 \\
   J003859  &     Fe I  & 5151.91 &    1.01  &   -3.32  & 38.82 & 0.82 & 5.31 & 10 \\
   J003859  &     Fe I  & 5166.28 &    0.00  &   -4.12  & 59.33 & 0.78 & 5.37 & 10 \\
   J003859  &     Fe I  & 5171.60 &    1.49  &   -1.72  & 83.20 & 0.75 & 5.13 & 10 \\
   J003859  &     Fe I  & 5191.45 &    3.04  &   -0.55  & 55.48 & 0.84 & 5.07 & 10 \\
   J003859  &     Fe I  & 5192.34 &    3.00  &   -0.42  & 62.14 & 0.79 & 5.02 & 10 \\
   J003859  &     Fe I  & 5194.94 &    1.56  &   -2.02  & 69.50 & 0.73 & 5.20 & 10 \\
   J003859  &     Fe I  & 5198.71 &    2.22  &   -2.09  & 26.13 & 0.75 & 5.15 & 10 \\
   J003859  &     Fe I  & 5202.34 &    2.18  &   -1.87  & 48.96 & 0.75 & 5.34 & 10 \\
   J003859  &     Fe I  & 5215.18 &    3.27  &   -0.86  & 21.41 & 0.73 & 4.95 & 9 \\
   J003859  &     Fe I  & 5216.27 &    1.61  &   -2.08  & 64.07 & 0.66 & 5.20 & 10 \\
   J003859  &     Fe I  & 5217.39 &    3.21  &   -1.07  & 21.27 & 0.70 & 5.09 & 9 \\
   J003859  &     Fe I  & 5225.53 &    0.11  &   -4.76  & 20.49 & 0.62 & 5.36 & 10 \\
   J003859  &     Fe I  & 5232.94 &    2.94  &   -0.06  & 82.20 & 0.67 & 4.99 & 10 \\
   J003859  &     Fe I  & 5242.49 &    3.63  &   -0.83  & 12.96 & 0.80 & 5.04 & 11 \\
   J003859  &     Fe I  & 5253.46 &    3.28  &   -1.58  & 13.16 & 1.61 & 5.42 & 9 \\
   J003859  &     Fe I  & 5263.31 &    3.27  &   -0.87  & 24.39 & 0.82 & 5.03 & 9 \\
   J003859  &     Fe I  & 5266.56 &    3.00  &   -0.38  & 62.16 & 0.81 & 4.98 & 10 \\
   J003859  &     Fe I  & 5281.79 &    3.04  &   -0.83  & 38.63 & 0.69 & 5.04 & 10 \\
   J003859  &     Fe I  & 5283.62 &    3.24  &   -0.45  & 46.52 & 0.68 & 5.02 & 9 \\
   J003859  &     Fe I  & 5307.36 &    1.61  &   -2.91  & 24.41 & 0.66 & 5.26 & 10 \\
   J003859  &     Fe I  & 5324.18 &    3.21  &   -0.11  & 66.09 & 0.73 & 5.00 & 12 \\
   J003859  &     Fe I  & 5332.90 &    1.56  &   -2.78  & 34.33 & 3.11 & 5.28 & 10 \\
   J003859  &     Fe I  & 5339.93 &    3.27  &   -0.63  & 37.09 & 0.94 & 5.05 & 9 \\
   J003859  &     Fe I  & 5341.02 &    1.61  &   -1.95  & 76.57 & 0.91 & 5.33 & 10 \\
   J003859  &     Fe I  & 5364.87 &    4.45  &    0.23  & 20.59 & 0.73 & 5.09 & 10 \\
   J003859  &     Fe I  & 5367.47 &    4.42  &    0.44  & 23.34 & 0.69 & 4.92 & 10 \\
   J003859  &     Fe I  & 5369.96 &    4.37  &    0.54  & 27.04 & 0.70 & 4.86 & 10 \\
   J003859  &     Fe I  & 5371.49 &    0.96  &   -1.64  & 119.93 & 0.62 & 5.30 & 10 \\
   J003859  &     Fe I  & 5383.37 &    4.31  &    0.64  & 35.77 & 0.65 & 4.88 & 10 \\
   J003859  &     Fe I  & 5397.13 &    0.92  &   -1.98  & 109.24 & 0.64 & 5.35 & 10 \\
   J003859  &     Fe I  & 5405.77 &    0.99  &   -1.85  & 108.90 & 0.65 & 5.29 & 10 \\
   J003859  &     Fe I  & 5410.91 &    4.47  &    0.40  & 26.19 & 2.00 & 5.08 & 10 \\
   J003859  &     Fe I  & 5415.20 &    4.39  &    0.64  & 33.80 & 0.83 & 4.92 & 10 \\
   J003859  &     Fe I  & 5429.70 &    0.96  &   -1.88  & 114.74 & 0.79 & 5.42 & 10 \\
   J003859  &     Fe I  & 5434.52 &    1.01  &   -2.13  & 98.68 & 0.77 & 5.35 & 10 \\
   J003859  &     Fe I  & 5497.52 &    1.01  &   -2.82  & 68.15 & 0.66 & 5.34 & 10 \\
   J003859  &     Fe I  & 5501.47 &    0.96  &   -3.05  & 60.39 & 0.70 & 5.36 & 10 \\
   J003859  &     Fe I  & 5569.62 &    3.42  &   -0.52  & 30.51 & 0.60 & 4.96 & 9 \\
   J003859  &     Fe I  & 5586.76 &    3.37  &   -0.11  & 54.31 & 0.67 & 4.95 & 9 \\
   J003859  &     Fe I  & 5624.54 &    3.42  &   -0.76  & 25.17 & 0.62 & 5.09 & 9 \\
   J003859  &     Fe I  & 6065.48 &    2.61  &   -1.41  & 35.33 & 0.63 & 5.05 & 10 \\
   J003859  &     Fe I  & 6136.61 &    2.45  &   -1.41  & 54.12 & 0.61 & 5.22 & 10 \\
   J003859  &     Fe I  & 6137.69 &    2.59  &   -1.35  & 45.88 & 0.61 & 5.17 & 10 \\
   J003859  &     Fe I  & 6191.56 &    2.43  &   -1.42  & 50.59 & 0.52 & 5.14 & 10 \\
   J003859  &     Fe I  & 6213.43 &    2.22  &   -2.48  & 13.73 & 0.58 & 5.15 & 10 \\
   J003859  &     Fe I  & 6219.28 &    2.20  &   -2.45  & 20.84 & 0.74 & 5.31 & 10 \\
   J003859  &     Fe I  & 6230.72 &    2.56  &   -1.28  & 57.47 & 0.68 & 5.27 & 10 \\
   J003859  &     Fe I  & 6246.32 &    3.60  &   -0.77  & 16.75 & 0.67 & 5.04 & 9 \\
   J003859  &     Fe I  & 6252.56 &    2.40  &   -1.77  & 43.62 & 0.63 & 5.33 & 10 \\
   J003859  &     Fe I  & 6265.13 &    2.18  &   -2.54  & 17.37 & 0.59 & 5.28 & 10 \\
   J003859  &     Fe I  & 6336.82 &    3.69  &   -0.85  & 11.87 & 0.80 & 5.04 & 9 \\
   J003859  &     Fe I  & 6393.60 &    2.43  &   -1.58  & 49.16 & 0.62 & 5.27 & 10 \\
   J003859  &     Fe I  & 6408.02 &    3.69  &   -0.99  & 9.32 & 0.75 & 5.06 & 9 \\
   J003859  &     Fe I  & 6411.65 &    3.65  &   -0.59  & 23.29 & 0.68 & 5.09 & 9 \\
   J003859  &     Fe I  & 6421.35 &    2.28  &   -2.01  & 34.44 & 0.45 & 5.26 & 10 \\
   J003859  &     Fe I  & 6494.98 &    2.40  &   -1.24  & 64.85 & 0.62 & 5.18 & 10 \\
   J003859  &     Fe I  & 6592.91 &    2.73  &   -1.47  & 29.90 & 0.69 & 5.11 & 10 \\
   J003859  &     Fe I  & 6593.87 &    2.43  &   -2.37  & 11.11 & 0.69 & 5.14 & 10 \\
   J003859  &     Fe I  & 7495.07 &    4.22  &   -0.10  & 20.51 & 0.89 & 5.11 & 12 \\
   J003859  &     Fe I  & 7511.02 &    4.18  &    0.12  & 29.89 & 0.82 & 5.07 & 9 \\
   J003859  &    Fe II  & 4178.86 &    2.58  &   -2.51  & 45.63 & 0.86 & 5.04 & 13 \\
   J003859  &    Fe II  & 4233.16 &    2.58  &   -2.02  & 72.43 & 1.00 & 5.09 & 14 \\
   J003859  &    Fe II  & 4416.82 &    2.78  &   -2.57  & 37.55 & 0.77 & 5.14 & 14 \\
   J003859  &    Fe II  & 4491.41 &    2.86  &   -2.71  & 25.02 & 0.76 & 5.10 & 13 \\
   J003859  &    Fe II  & 4508.28 &    2.86  &   -2.42  & 44.83 & 0.85 & 5.21 & 14 \\
   J003859  &    Fe II  & 4515.34 &    2.84  &   -2.60  & 33.60 & 0.71 & 5.15 & 13 \\
   J003859  &    Fe II  & 4555.89 &    2.83  &   -2.40  & 42.84 & 0.69 & 5.12 & 13 \\
   J003859  &    Fe II  & 4576.34 &    2.84  &   -2.95  & 18.16 & 0.81 & 5.13 & 13 \\
   J003859  &    Fe II  & 4583.83 &    2.81  &   -1.94  & 67.55 & 0.72 & 5.11 & 14 \\
   J003859  &    Fe II  & 4620.52 &    2.83  &   -3.21  & 10.18 & 1.43 & 5.08 & 13 \\
   J003859  &    Fe II  & 5197.58 &    3.23  &   -2.22  & 32.37 & 0.75 & 5.12 & 13 \\
   J003859  &    Fe II  & 5234.63 &    3.22  &   -2.18  & 35.20 & 0.70 & 5.13 & 13 \\
   J003859  &    Fe II  & 5276.00 &    3.20  &   -2.01  & 43.01 & 0.74 & 5.08 & 13 \\
   J003859  &     Ni I  & 3807.14 &    0.42  &   -1.23  & 98.17 & 1.43 & 3.89 & 15 \\
   J003859  &     Ni I  & 4470.48 &    3.40  &   -0.30  & 10.95 & 0.77 & 3.91 & 15 \\
   J003859  &     Ni I  & 4604.99 &    3.48  &   -0.24  & 12.30 & 0.92 & 3.98 & 15 \\
   J003859  &     Ni I  & 4686.22 &    3.60  &   -0.59  & 3.43 & 0.73 & 3.86 & 15 \\
   J003859  &     Ni I  & 4714.42 &    3.38  &    0.25  & 27.76 & 0.72 & 3.83 & 15 \\
   J003859  &     Ni I  & 4756.52 &    3.48  &   -0.27  & 9.72 & 0.98 & 3.89 & 15 \\
   J003859  &     Ni I  & 4904.41 &    3.54  &   -0.17  & 12.64 & 0.86 & 3.98 & 1 \\
   J003859  &     Ni I  & 4980.17 &    3.60  &    0.07  & 11.94 & 0.76 & 3.77 & 15 \\
   J003859  &     Ni I  & 5017.58 &    3.54  &   -0.03  & 14.59 & 1.48 & 3.90 & 15 \\
   J003859  &     Ni I  & 5080.53 &    3.65  &    0.32  & 17.79 & 0.76 & 3.77 & 15 \\
   J003859  &     Ni I  & 5081.11 &    3.85  &    0.30  & 14.48 & 0.71 & 3.90 & 1 \\
   J003859  &     Ni I  & 5084.08 &    3.68  &    0.03  & 10.73 & 0.77 & 3.84 & 1 \\
   J003859  &     Ni I  & 5115.40 &    3.83  &   -0.11  & 5.31 & 0.74 & 3.80 & 1 \\
   J003859  &     Ni I  & 5476.90 &    1.83  &   -0.78  & 66.25 & 0.69 & 3.88 & 15 \\
   J003859  &     Ni I  & 6643.63 &    1.68  &   -2.22  & 12.38 & 0.63 & 3.91 & 15 \\
   J003859  &     Zn I  & 4722.16 &    4.03  &   -0.37  & 14.38 & 0.79 & 2.42 & 16 \\
   J003859  &     Zn I  & 4810.54 &    4.08  &   -0.15  & 16.48 & 0.69 & 2.32 & 16 \\
   J003859  &    C-H I  & 4312.00 &     NaN  &     NaN  &     synth  &    synth  & 6.54 & NaN \\
   J003859  &    C-H I  & 4323.00 &     NaN  &     NaN  &     synth  &    synth  & 6.48 & NaN \\
   J003859  &    C-H I  & 4230.00 &     NaN  &     NaN  &     synth  &    synth  & 6.53 & NaN \\
   J003859  &    C-H I  & 4311.00 &     NaN  &     NaN  &     synth  &    synth  & 6.50 & NaN \\
   J003859  &     Li I  & 6707.80 &    0.00  &    0.17  &     synth  &    synth  & 1.04 & 17 \\
   J003859  &     Al I  & 3944.00 &    0.00  &   -0.64  &     synth  &    synth  & 3.42 & 1 \\
   J003859  &     Si I  & 4102.94 &    1.91  &   -3.34  &     synth  &    synth  & 5.98 & 1 \\
   J003859  &    Sc II  & 4246.82 &    0.32  &    0.24  &     synth  &    synth  & 1.00 & 18 \\
   J003859  &    Sc II  & 4324.99 &    0.60  &   -0.44  &     synth  &    synth  & 0.86 & 18 \\
   J003859  &    Sc II  & 4374.47 &    0.62  &   -0.46  &     synth  &    synth  & 0.90 & 18 \\
   J003859  &    Sc II  & 4400.39 &    0.61  &   -0.54  &     synth  &    synth  & 0.89 & 18 \\
   J003859  &    Sc II  & 4415.56 &    0.60  &   -0.68  &     synth  &    synth  & 0.88 & 18 \\
   J003859  &    Sc II  & 5031.02 &    1.36  &   -0.41  &     synth  &    synth  & 0.94 & 18 \\
   J003859  &    Sc II  & 5526.79 &    1.77  &   -0.01  &     synth  &    synth  & 0.81 & 18 \\
   J003859  &    Sc II  & 5657.90 &    1.51  &   -0.54  &     synth  &    synth  & 0.98 & 18 \\
   J003859  &      V I  & 4111.78 &    0.30  &    0.40  &     synth  &    synth  & 1.55 & 19 \\
   J003859  &      V I  & 4379.23 &    0.30  &    0.58  &     synth  &    synth  & 1.59 & 19 \\
   J003859  &     V II  & 3715.46 &    1.57  &   -0.22  &     synth  &    synth  & 1.65 & 20 \\
   J003859  &     V II  & 3727.34 &    1.69  &   -0.23  &     synth  &    synth  & 1.79 & 20 \\
   J003859  &     V II  & 3903.25 &    1.48  &   -0.91  &     synth  &    synth  & 1.86 & 20 \\
   J003859  &     V II  & 4002.93 &    1.43  &   -1.44  &     synth  &    synth  & 1.86 & 20 \\
   J003859  &     V II  & 4002.93 &    1.43  &   -1.44  &     synth  &    synth  & 1.76 & 20 \\
   J003859  &     V II  & 4023.38 &    1.80  &   -0.61  &     synth  &    synth  & 1.75 & 20 \\
   J003859  &     Mn I  & 4030.75 &    0.00  &   -0.50  &     synth  &    synth  & 2.98 & 21 \\
   J003859  &     Mn I  & 4033.06 &    0.00  &   -0.65  &     synth  &    synth  & 2.80 & 21 \\
   J003859  &     Mn I  & 4034.48 &    0.00  &   -0.84  &     synth  &    synth  & 2.72 & 21 \\
   J003859  &     Mn I  & 4041.35 &    2.11  &    0.28  &     synth  &    synth  & 2.62 & 21 \\
   J003859  &     Mn I  & 4754.04 &    2.28  &   -0.08  &     synth  &    synth  & 2.64 & 21 \\
   J003859  &     Mn I  & 4823.52 &    2.32  &    0.14  &     synth  &    synth  & 2.72 & 21 \\
   J003859  &     Co I  & 3842.05 &    0.92  &   -0.74  &     synth  &    synth  & 2.77 & 22 \\
   J003859  &     Co I  & 3845.47 &    0.92  &    0.06  &     synth  &    synth  & 2.67 & 22 \\
   J003859  &     Co I  & 3894.08 &    1.05  &    0.12  &     synth  &    synth  & 2.55 & 22 \\
   J003859  &     Co I  & 3995.31 &    0.92  &   -0.18  &     synth  &    synth  & 2.60 & 22 \\
   J003859  &     Co I  & 4118.77 &    1.05  &   -0.48  &     synth  &    synth  & 2.81 & 22 \\
   J003859  &     Co I  & 4121.32 &    0.92  &   -0.33  &     synth  &    synth  & 2.92 & 22 \\
   J003859  &    Sr II  & 4077.71 &    0.00  &    0.15  &     synth  &    synth  & 0.81 & 23 \\
   J003859  &    Sr II  & 4215.52 &    0.00  &   -0.17  &     synth  &    synth  & 0.78 & 23 \\
   J003859  &     Y II  & 3710.29 &    0.18  &    0.51  &     synth  &    synth  & -0.36 & 24 \\
   J003859  &     Y II  & 3747.55 &    0.10  &   -0.95  &     synth  &    synth  & 0.01 & 24 \\
   J003859  &     Y II  & 3774.33 &    0.13  &    0.29  &     synth  &    synth  & -0.15 & NaN \\
   J003859  &     Y II  & 3832.89 &    0.18  &   -0.34  &     synth  &    synth  & -0.24 & 24 \\
   J003859  &     Y II  & 3982.59 &    0.13  &   -0.56  &     synth  &    synth  & -0.09 & 24 \\
   J003859  &     Y II  & 4235.73 &    0.13  &   -1.27  &     synth  &    synth  & -0.26 & 24 \\
   J003859  &     Y II  & 4358.72 &    0.10  &   -1.15  &     synth  &    synth  & -0.40 & 24 \\
   J003859  &     Y II  & 4883.68 &    1.08  &    0.19  &     synth  &    synth  & -0.30 & 24 \\
   J003859  &     Y II  & 4900.12 &    1.03  &    0.03  &     synth  &    synth  & -0.40 & 24 \\
   J003859  &     Y II  & 5087.42 &    1.08  &   -0.16  &     synth  &    synth  & -0.42 & 24 \\
   J003859  &     Y II  & 5200.41 &    0.99  &   -0.47  &     synth  &    synth  & -0.34 & 24 \\
   J003859  &    Zr II  & 3766.82 &    0.41  &   -0.83  &     synth  &    synth  & 0.60 & 25 \\
   J003859  &    Zr II  & 3998.96 &    0.56  &   -0.52  &     synth  &    synth  & 0.64 & 25 \\
   J003859  &    Zr II  & 4050.32 &    0.71 &    -1.06  &     synth  &    synth  & 0.49 & 25 \\
   J003859  &    Zr II  & 4149.20 &    0.80  &   -0.04  &     synth  &    synth  & 0.48 & 25 \\
   J003859  &    Zr II  & 4161.20 &    0.71 &    -0.59  &     synth  &    synth  & 0.52 & 25 \\
   J003859  &    Zr II  & 4208.98 &    0.71  &   -0.51  &     synth  &    synth  & 0.60 & 25 \\
   J003859  &    Zr II  & 4211.88 &    0.53  &    -1.04  &     synth  &    synth  & 0.68 & 25 \\
   J003859  &    Zr II  & 4258.04 &    0.56  &   -1.20  &     synth  &    synth  & 0.66 & 25 \\
   J003859  &    Ba II  & 4554.03 &    0.00  &    0.14  &     synth  &    synth  & -0.58 & 26 \\
   J003859  &    Ba II  & 4934.08 &    0.00  &   -0.16  &     synth  &    synth  & -0.61 & 26 \\
   J003859  &    Ba II  & 5853.68 &    0.60  &   -0.91  &     synth  &    synth  & -0.56 & 26 \\
   J003859  &    Ba II  & 6141.71 &    0.70  &   -0.03  &     synth  &    synth  & -0.56 & 26 \\
   J003859  &    Ba II  & 6496.90 &    0.60  &   -0.41  &     synth  &    synth  & -0.58 & 26 \\
   J003859  &    La II  & 3794.77 &    0.24  &    0.21  &     synth  &    synth  & -1.55 & 27 \\
   J003859  &    La II  & 4077.34 &    0.24  &   -0.06  &     synth  &    synth  & -1.23 & 27 \\
   J003859  &    La II  & 4123.22 &    0.32  &    0.13  &     synth  &    synth  & -1.30 & 27 \\
   J003859  &    Nd II  & 4109.45 &    0.32  &    0.35  &     synth  &    synth  & -0.86 & 28 \\
   J003859  &    Nd II  & 4303.57 &    0.00  &    0.08  &     synth  &    synth  & -0.81 & 28 \\
   J003859  &    Eu II  & 3819.67 &    0.00  &    0.51  &     synth  &    synth  & -1.75 & 29 \\
   J003859  &    Eu II  & 4129.72 &    0.00  &    0.22  &     synth  &    synth  & -1.71 & 29 \\
   J003859  &    Eu II  & 4205.04 &    0.00  &    0.21  &     synth  &    synth  & -1.74 & 29 \\
   J003859  &    Dy II  & 3944.68 &    0.00  &    0.11  &     synth  &    synth  & -1.37 & 30 \\
   J003859  &    Dy II  & 4077.97 &    0.10  &   -0.04  &     synth  &    synth  & -1.22 & 30 \\
   J003859  &    Er II  & 3906.31 &    0.00  &    0.12  &     synth  &    synth  & -1.18 & 31 \\
   J003859  &    Yb II  & 3694.19 &    0.00  &   -0.30  &     synth  &    synth  & -1.63 & 32 \\
 J20313531  &      O I  & 7771.94 &    9.15  &    0.37  & 13.36 & 0.94 & 7.46 & 1 \\
 J20313531  &      O I  & 7774.17 &    9.15  &    0.22  & 12.55 & 1.40 & 7.57 & 1 \\
 J20313531  &     Na I  & 5889.95 &    0.00  &    0.11  & 172.03 & 0.93 & 4.20 & 1 \\
 J20313531  &     Na I  & 5895.92 &    0.00  &   -0.19  & 151.52 & 0.97 & 4.26 & 1 \\
 J20313531  &     Na I  & 8194.81 &    2.10  &    0.54  & 69.30 & 1.15 & 4.33 & 1 \\
 J20313531  &     Mg I  & 3829.35 &    2.71  &   -0.23  & 187.34 & 1.48 & 5.40 & 1 \\
 J20313531  &     Mg I  & 4167.27 &    4.35  &   -0.74  & 68.87 & 1.00 & 5.78 & 1 \\
 J20313531  &     Mg I  & 4702.99 &    4.33  &   -0.44  & 84.55 & 0.71 & 5.60 & 1 \\
 J20313531  &     Mg I  & 5172.68 &    2.71  &   -0.36  & 224.08 & 1.67 & 5.51 & 2 \\
 J20313531  &     Mg I  & 5183.60 &    2.72  &   -0.17  & 261.96 & 1.80 & 5.52 & 2 \\
 J20313531  &     Mg I  & 5528.40 &    4.35  &   -0.55  & 88.90 & 1.14 & 5.82 & 2 \\
 J20313531  &     Mg I  & 5711.09 &    4.35  &   -1.84  & 16.78 & 1.17 & 5.87 & 2 \\
 J20313531  &     Al I  & 3944.00 &    0.00  &   -0.64  & 202.15 & 1.79 & 4.52 & 1 \\
 J20313531  &     Si I  & 3905.52 &    1.91  &   -1.04  & 240.17 & 1.82 & 5.65 & 1 \\
 J20313531  &     Si I  & 5948.54 &    5.08  &   -1.23  & 5.97 & 0.89 & 5.50 & 1 \\
 J20313531  &     Si I  & 7742.72 &    6.21  &   -0.28  & 6.81 & 0.85 & 5.75 & 1 \\
 J20313531  &     Si I  & 7944.00 &    5.98  &   -0.31  & 9.02 & 1.05 & 5.66 & 1 \\
 J20313531  &      K I  & 7664.90 &    0.00  &    0.12  & 74.40 & 0.89 & 3.55 & 1 \\
 J20313531  &      K I  & 7698.96 &    0.00  &   -0.18  & 51.06 & 1.10 & 3.44 & 1 \\
 J20313531  &     Ca I  & 4318.65 &    1.90  &   -0.21  & 65.97 & 0.77 & 4.40 & 1 \\
 J20313531  &     Ca I  & 4355.08 &    2.71  &   -0.42  & 15.34 & 0.72 & 4.39 & 1 \\
 J20313531  &     Ca I  & 4425.44 &    1.88  &   -0.41  & 58.80 & 0.72 & 4.41 & 3 \\
 J20313531  &     Ca I  & 4435.69 &    1.89  &   -0.55  & 55.05 & 0.78 & 4.50 & 3 \\
 J20313531  &     Ca I  & 4454.78 &    1.90  &    0.26  & 88.81 & 0.74 & 4.34 & 1 \\
 J20313531  &     Ca I  & 4455.89 &    1.90  &   -0.55  & 53.79 & 0.74 & 4.48 & 3 \\
 J20313531  &     Ca I  & 4456.61 &    1.90  &   -1.74  & 9.39 & 0.65 & 4.61 & 3 \\
 J20313531  &     Ca I  & 4526.94 &    2.71  &   -0.47  & 14.74 & 0.80 & 4.41 & 3 \\
 J20313531  &     Ca I  & 4578.55 &    2.52  &   -0.67  & 12.27 & 0.69 & 4.32 & 3 \\
 J20313531  &     Ca I  & 5261.71 &    2.52  &   -0.60  & 18.54 & 1.24 & 4.44 & 3 \\
 J20313531  &     Ca I  & 5512.98 &    2.93  &   -0.45  & 12.16 & 1.31 & 4.49 & 3 \\
 J20313531  &     Ca I  & 5581.97 &    2.52  &   -0.58  & 17.61 & 1.25 & 4.38 & 3 \\
 J20313531  &     Ca I  & 5588.76 &    2.52  &    0.30  & 61.02 & 1.01 & 4.40 & 3 \\
 J20313531  &     Ca I  & 5590.12 &    2.52  &   -0.60  & 20.60 & 1.05 & 4.48 & 3 \\
 J20313531  &     Ca I  & 5601.29 &    2.53  &   -0.57  & 21.94 & 1.08 & 4.50 & 3 \\
 J20313531  &     Ca I  & 5857.45 &    2.93  &    0.17  & 38.01 & 1.12 & 4.53 & 3 \\
 J20313531  &     Ca I  & 6102.72 &    1.88  &   -0.81  & 45.80 & 0.91 & 4.50 & 3 \\
 J20313531  &     Ca I  & 6122.22 &    1.89  &   -0.33  & 75.67 & 1.01 & 4.55 & 3 \\
 J20313531  &     Ca I  & 6161.29 &    2.52  &   -1.35  & 4.99 & 0.94 & 4.52 & 3 \\
 J20313531  &     Ca I  & 6162.17 &    1.90  &   -0.11  & 86.11 & 0.92 & 4.52 & 3 \\
 J20313531  &     Ca I  & 6166.44 &    2.52  &   -1.22  & 6.39 & 1.03 & 4.50 & 3 \\
 J20313531  &     Ca I  & 6169.06 &    2.52  &   -0.87  & 15.50 & 1.04 & 4.58 & 3 \\
 J20313531  &     Ca I  & 6169.56 &    2.53  &   -0.60  & 25.50 & 0.96 & 4.59 & 3 \\
 J20313531  &     Ca I  & 6439.07 &    2.52  &    0.33  & 69.80 & 0.82 & 4.50 & 3 \\
 J20313531  &     Ca I  & 6449.81 &    2.52  &   -0.55  & 26.45 & 0.90 & 4.55 & 3 \\
 J20313531  &     Ca I  & 6455.60 &    2.52  &   -1.42  & 4.75 & 0.89 & 4.55 & 3 \\
 J20313531  &     Ca I  & 6471.66 &    2.53  &   -0.71  & 20.90 & 1.07 & 4.59 & 3 \\
 J20313531  &     Ca I  & 6499.65 &    2.52  &   -0.81  & 17.69 & 1.03 & 4.58 & 3 \\
 J20313531  &     Ti I  & 3989.76 &    0.02  &   -0.13  & 67.68 & 0.97 & 3.02 & 4 \\
 J20313531  &     Ti I  & 3998.64 &    0.05  &    0.02  & 69.48 & 0.92 & 2.94 & 4 \\
 J20313531  &     Ti I  & 4512.73 &    0.84  &   -0.40  & 17.95 & 0.66 & 3.07 & 4 \\
 J20313531  &     Ti I  & 4518.02 &    0.83  &   -0.25  & 20.39 & 0.76 & 2.97 & 4 \\
 J20313531  &     Ti I  & 4533.24 &    0.85  &    0.54  & 54.39 & 0.72 & 2.90 & 4 \\
 J20313531  &     Ti I  & 4534.78 &    0.84  &    0.35  & 44.19 & 0.69 & 2.89 & 4 \\
 J20313531  &     Ti I  & 4548.76 &    0.83  &   -0.28  & 18.76 & 0.70 & 2.96 & 4 \\
 J20313531  &     Ti I  & 4555.48 &    0.85  &   -0.40  & 13.03 & 0.74 & 2.91 & 4 \\
 J20313531  &     Ti I  & 4656.47 &    0.00  &   -1.28  & 19.02 & 0.65 & 3.05 & 1 \\
 J20313531  &     Ti I  & 4681.91 &    0.05  &   -1.01  & 24.68 & 0.66 & 2.98 & 1 \\
 J20313531  &     Ti I  & 4840.87 &    0.90  &   -0.43  & 12.17 & 0.86 & 2.94 & 4 \\
 J20313531  &     Ti I  & 4981.73 &    0.84  &    0.57  & 57.65 & 0.77 & 2.88 & 4 \\
 J20313531  &     Ti I  & 4999.50 &    0.83  &    0.32  & 48.12 & 0.92 & 2.94 & 4 \\
 J20313531  &     Ti I  & 5016.16 &    0.85  &   -0.48  & 14.93 & 0.91 & 3.02 & 4 \\
 J20313531  &     Ti I  & 5064.65 &    0.05  &   -0.94  & 32.35 & 1.36 & 3.04 & 4 \\
 J20313531  &     Ti I  & 5173.74 &    0.00  &   -1.06  & 29.71 & 1.42 & 3.05 & 4 \\
 J20313531  &     Ti I  & 5192.97 &    0.02  &   -0.95  & 35.93 & 1.50 & 3.08 & 4 \\
 J20313531  &     Ti I  & 5210.38 &    0.05  &   -0.82  & 39.66 & 1.42 & 3.06 & 4 \\
 J20313531  &    Ti II  & 3491.05 &    0.11  &   -1.10  & 118.17 & 2.76 & 3.32 & 5 \\
 J20313531  &    Ti II  & 3759.29 &    0.61  &    0.28  & 173.94 & 1.76 & 3.13 & 5 \\
 J20313531  &    Ti II  & 3761.32 &    0.57  &    0.18  & 166.26 & 1.51 & 3.11 & 5 \\
 J20313531  &    Ti II  & 4028.34 &    1.89  &   -0.92  & 50.31 & 0.94 & 2.99 & 5 \\
 J20313531  &    Ti II  & 4394.06 &    1.22  &   -1.77  & 50.43 & 0.77 & 3.06 & 5 \\
 J20313531  &    Ti II  & 4395.84 &    1.24  &   -1.93  & 36.84 & 0.65 & 2.99 & 5 \\
 J20313531  &    Ti II  & 4399.77 &    1.24  &   -1.20  & 83.92 & 0.72 & 3.24 & 5 \\
 J20313531  &    Ti II  & 4409.52 &    1.23  &   -2.53  & 14.60 & 0.68 & 3.04 & 5 \\
 J20313531  &    Ti II  & 4417.71 &    1.17  &   -1.19  & 81.68 & 0.72 & 3.09 & 6 \\
 J20313531  &    Ti II  & 4418.33 &    1.24  &   -1.99  & 42.15 & 0.80 & 3.15 & 5 \\
 J20313531  &    Ti II  & 4443.80 &    1.08  &   -0.71  & 102.89 & 0.70 & 3.05 & 5 \\
 J20313531  &    Ti II  & 4444.55 &    1.12  &   -2.20  & 38.01 & 0.81 & 3.15 & 5 \\
 J20313531  &    Ti II  & 4450.48 &    1.08  &   -1.52  & 70.37 & 0.70 & 3.05 & 5 \\
 J20313531  &    Ti II  & 4464.45 &    1.16  &   -1.81  & 55.94 & 0.82 & 3.13 & 6 \\
 J20313531  &    Ti II  & 4470.85 &    1.17  &   -2.02  & 37.35 & 0.72 & 3.00 & 6 \\
 J20313531  &    Ti II  & 4493.52 &    1.08  &   -2.78  & 13.83 & 0.74 & 3.09 & 5 \\
 J20313531  &    Ti II  & 4501.27 &    1.12  &   -0.77  & 100.72 & 0.73 & 3.08 & 5 \\
 J20313531  &    Ti II  & 4533.96 &    1.24  &   -0.53  & 106.69 & 0.78 & 3.12 & 6 \\
 J20313531  &    Ti II  & 4571.97 &    1.57  &   -0.31  & 96.50 & 0.69 & 2.99 & 5 \\
 J20313531  &    Ti II  & 4583.41 &    1.16  &   -2.84  & 11.82 & 1.41 & 3.15 & 5 \\
 J20313531  &    Ti II  & 4708.66 &    1.24  &   -2.35  & 26.05 & 0.69 & 3.16 & 5 \\
 J20313531  &    Ti II  & 4798.53 &    1.08  &   -2.66  & 22.26 & 3.43 & 3.20 & 5 \\
 J20313531  &    Ti II  & 5129.16 &    1.89  &   -1.34  & 38.56 & 1.64 & 3.09 & 5 \\
 J20313531  &    Ti II  & 5185.90 &    1.89  &   -1.41  & 33.78 & 1.41 & 3.06 & 5 \\
 J20313531  &    Ti II  & 5336.79 &    1.58  &   -1.60  & 43.56 & 1.26 & 3.09 & 5 \\
 J20313531  &    Ti II  & 5381.02 &    1.57  &   -1.97  & 29.87 & 1.26 & 3.18 & 5 \\
 J20313531  &    Ti II  & 5418.77 &    1.58  &   -2.13  & 20.59 & 1.20 & 3.13 & 5 \\
 J20313531  &     Cr I  & 4289.72 &    0.00  &   -0.37  & 93.79 & 0.76 & 3.04 & 7 \\
 J20313531  &     Cr I  & 4545.95 &    0.94  &   -1.37  & 16.86 & 0.78 & 3.29 & 7 \\
 J20313531  &     Cr I  & 4646.15 &    1.03  &   -0.74  & 37.86 & 0.76 & 3.25 & 7 \\
 J20313531  &     Cr I  & 4651.28 &    0.98  &   -1.46  & 13.29 & 0.71 & 3.30 & 7 \\
 J20313531  &     Cr I  & 5206.04 &    0.94  &    0.02  & 82.16 & 1.32 & 3.23 & 7 \\
 J20313531  &     Cr I  & 5296.69 &    0.98  &   -1.36  & 16.18 & 1.16 & 3.26 & 7 \\
 J20313531  &     Cr I  & 5348.31 &    1.00  &   -1.21  & 17.63 & 1.25 & 3.17 & 7 \\
 J20313531  &    Cr II  & 4558.64 &    4.07  &   -0.43  & 24.10 & 0.79 & 3.37 & 8 \\
 J20313531  &    Cr II  & 4588.20 &    4.07  &   -0.65  & 18.32 & 0.69 & 3.43 & 8 \\
 J20313531  &    Cr II  & 4618.81 &    4.07  &   -0.89  & 15.33 & 0.91 & 3.57 & 8 \\
 J20313531  &     Fe I  & 3742.62 &    2.94  &   -0.81  & 46.90 & 1.70 & 5.22 & 9 \\
 J20313531  &     Fe I  & 3786.68 &    1.01  &   -2.18  & 71.22 & 1.17 & 5.07 & 10 \\
 J20313531  &     Fe I  & 3808.73 &    2.56  &   -1.17  & 47.76 & 1.21 & 5.19 & 11 \\
 J20313531  &     Fe I  & 3902.95 &    1.56  &   -0.44  & 121.05 & 1.18 & 5.07 & 10 \\
 J20313531  &     Fe I  & 3949.95 &    2.18  &   -1.25  & 59.02 & 0.97 & 5.08 & 10 \\
 J20313531  &     Fe I  & 4067.98 &    3.21  &   -0.53  & 46.01 & 0.83 & 5.17 & 9 \\
 J20313531  &     Fe I  & 4070.77 &    3.24  &   -0.87  & 30.62 & 0.93 & 5.23 & 9 \\
 J20313531  &     Fe I  & 4132.06 &    1.61  &   -0.68  & 118.79 & 0.93 & 5.27 & 10 \\
 J20313531  &     Fe I  & 4143.87 &    1.56  &   -0.51  & 118.88 & 0.78 & 5.04 & 10 \\
 J20313531  &     Fe I  & 4147.67 &    1.49  &   -2.07  & 64.19 & 0.80 & 5.23 & 10 \\
 J20313531  &     Fe I  & 4157.78 &    3.42  &   -0.40  & 42.38 & 0.85 & 5.19 & 10 \\
 J20313531  &     Fe I  & 4158.79 &    3.43  &   -0.70  & 24.69 & 0.93 & 5.12 & 9 \\
 J20313531  &     Fe I  & 4182.38 &    3.02  &   -1.18  & 23.55 & 0.85 & 5.14 & 10 \\
 J20313531  &     Fe I  & 4184.89 &    2.83  &   -0.87  & 47.24 & 0.81 & 5.13 & 10 \\
 J20313531  &     Fe I  & 4187.04 &    2.45  &   -0.56  & 81.33 & 0.78 & 5.11 & 12 \\
 J20313531  &     Fe I  & 4199.10 &    3.05  &    0.16  & 79.68 & 0.80 & 5.07 & 10 \\
 J20313531  &     Fe I  & 4216.18 &    0.00  &   -3.36  & 86.37 & 0.82 & 5.43 & 10 \\
 J20313531  &     Fe I  & 4217.55 &    3.43  &   -0.48  & 34.28 & 0.79 & 5.11 & 10 \\
 J20313531  &     Fe I  & 4222.21 &    2.45  &   -0.91  & 66.14 & 0.85 & 5.12 & 10 \\
 J20313531  &     Fe I  & 4233.60 &    2.48  &   -0.60  & 77.99 & 0.80 & 5.09 & 12 \\
 J20313531  &     Fe I  & 4238.81 &    3.40  &   -0.23  & 47.13 & 0.83 & 5.08 & 10 \\
 J20313531  &     Fe I  & 4250.12 &    2.47  &   -0.38  & 85.72 & 0.71 & 5.03 & 10 \\
 J20313531  &     Fe I  & 4250.79 &    1.56  &   -0.71  & 109.74 & 0.73 & 5.04 & 10 \\
 J20313531  &     Fe I  & 4415.12 &    1.61  &   -0.62  & 120.85 & 0.74 & 5.17 & 10 \\
 J20313531  &     Fe I  & 4430.61 &    2.22  &   -1.73  & 46.45 & 0.71 & 5.28 & 10 \\
 J20313531  &     Fe I  & 4442.34 &    2.20  &   -1.23  & 74.38 & 0.78 & 5.32 & 10 \\
 J20313531  &     Fe I  & 4443.19 &    2.86  &   -1.04  & 39.82 & 0.71 & 5.16 & 10 \\
 J20313531  &     Fe I  & 4447.72 &    2.22  &   -1.36  & 64.88 & 0.73 & 5.27 & 11 \\
 J20313531  &     Fe I  & 4461.65 &    0.09  &   -3.19  & 88.33 & 0.68 & 5.35 & 10 \\
 J20313531  &     Fe I  & 4466.55 &    2.83  &   -0.60  & 69.87 & 0.67 & 5.31 & 10 \\
 J20313531  &     Fe I  & 4484.22 &    3.60  &   -0.64  & 18.23 & 0.71 & 5.05 & 9 \\
 J20313531  &     Fe I  & 4489.74 &    0.12  &   -3.90  & 57.23 & 0.74 & 5.35 & 10 \\
 J20313531  &     Fe I  & 4494.56 &    2.20  &   -1.14  & 75.00 & 0.74 & 5.24 & 10 \\
 J20313531  &     Fe I  & 4547.85 &    3.55  &   -0.82  & 17.21 & 0.67 & 5.14 & 11 \\
 J20313531  &     Fe I  & 4592.65 &    1.56  &   -2.46  & 55.13 & 0.76 & 5.44 & 10 \\
 J20313531  &     Fe I  & 4602.00 &    1.61  &   -3.13  & 17.16 & 0.80 & 5.35 & 10 \\
 J20313531  &     Fe I  & 4602.94 &    1.49  &   -2.21  & 65.49 & 0.69 & 5.34 & 10 \\
 J20313531  &     Fe I  & 4607.65 &    3.27  &   -1.33  & 15.00 & 0.82 & 5.28 & 9 \\
 J20313531  &     Fe I  & 4619.29 &    3.60  &   -1.06  & 11.76 & 0.63 & 5.24 & 9 \\
 J20313531  &     Fe I  & 4630.12 &    2.28  &   -2.58  & 14.16 & 0.75 & 5.43 & 11 \\
 J20313531  &     Fe I  & 4643.46 &    3.65  &   -1.15  & 10.55 & 0.80 & 5.32 & 10 \\
 J20313531  &     Fe I  & 4647.43 &    2.95  &   -1.35  & 28.07 & 0.72 & 5.31 & 10 \\
 J20313531  &     Fe I  & 4668.13 &    3.27  &   -1.08  & 23.75 & 0.83 & 5.28 & 9 \\
 J20313531  &     Fe I  & 4733.59 &    1.49  &   -2.99  & 29.95 & 0.70 & 5.39 & 10 \\
 J20313531  &     Fe I  & 4736.77 &    3.21  &   -0.67  & 44.23 & 0.71 & 5.22 & 9 \\
 J20313531  &     Fe I  & 4789.65 &    3.55  &   -0.96  & 17.10 & 0.97 & 5.27 & 10 \\
 J20313531  &     Fe I  & 4871.32 &    2.87  &   -0.34  & 72.88 & 0.79 & 5.06 & 12 \\
 J20313531  &     Fe I  & 4872.14 &    2.88  &   -0.57  & 63.58 & 0.78 & 5.12 & 10 \\
 J20313531  &     Fe I  & 4890.76 &    2.88  &   -0.38  & 71.27 & 0.73 & 5.08 & 12 \\
 J20313531  &     Fe I  & 4891.49 &    2.85  &   -0.11  & 87.18 & 0.69 & 5.10 & 10 \\
 J20313531  &     Fe I  & 4910.02 &    3.40  &   -1.28  & 9.59 & 0.65 & 5.13 & 9 \\
 J20313531  &     Fe I  & 4920.50 &    2.83  &    0.07  & 97.52 & 0.81 & 5.10 & 10 \\
 J20313531  &     Fe I  & 4924.77 &    2.28  &   -2.11  & 21.63 & 0.80 & 5.17 & 10 \\
 J20313531  &     Fe I  & 4938.81 &    2.88  &   -1.08  & 40.92 & 0.83 & 5.20 & 10 \\
 J20313531  &     Fe I  & 4939.69 &    0.86  &   -3.25  & 48.81 & 0.78 & 5.31 & 10 \\
 J20313531  &     Fe I  & 4946.39 &    3.37  &   -1.11  & 15.51 & 0.75 & 5.16 & 12 \\
 J20313531  &     Fe I  & 4950.11 &    3.42  &   -1.50  & 8.47 & 0.93 & 5.31 & 9 \\
 J20313531  &     Fe I  & 4994.13 &    0.92  &   -2.97  & 60.68 & 0.88 & 5.32 & 10 \\
 J20313531  &     Fe I  & 5001.86 &    3.88  &   -0.01  & 35.80 & 0.97 & 5.10 & 12 \\
 J20313531  &     Fe I  & 5002.79 &    3.40  &   -1.46  & 6.77 & 1.05 & 5.14 & 12 \\
 J20313531  &     Fe I  & 5006.12 &    2.83  &   -0.62  & 63.46 & 0.88 & 5.10 & 10 \\
 J20313531  &     Fe I  & 5014.94 &    3.94  &   -0.18  & 22.73 & 0.78 & 5.05 & 9 \\
 J20313531  &     Fe I  & 5022.24 &    3.98  &   -0.33  & 13.64 & 0.80 & 4.96 & 12 \\
 J20313531  &     Fe I  & 5049.82 &    2.28  &   -1.36  & 60.12 & 1.15 & 5.19 & 10 \\
 J20313531  &     Fe I  & 5051.63 &    0.92  &   -2.76  & 73.40 & 1.01 & 5.38 & 10 \\
 J20313531  &     Fe I  & 5068.77 &    2.94  &   -1.04  & 41.90 & 1.63 & 5.23 & 10 \\
 J20313531  &     Fe I  & 5083.34 &    0.96  &   -2.84  & 61.34 & 1.35 & 5.24 & 10 \\
 J20313531  &     Fe I  & 5123.72 &    1.01  &   -3.06  & 56.28 & 1.50 & 5.42 & 10 \\
 J20313531  &     Fe I  & 5127.36 &    0.92  &   -3.25  & 47.49 & 1.41 & 5.34 & 10 \\
 J20313531  &     Fe I  & 5131.47 &    2.22  &   -2.52  & 21.57 & 1.63 & 5.50 & 10 \\
 J20313531  &     Fe I  & 5133.69 &    4.18  &    0.36  & 39.38 & 1.27 & 5.12 & 9 \\
 J20313531  &     Fe I  & 5150.84 &    0.99  &   -3.04  & 47.34 & 1.29 & 5.20 & 10 \\
 J20313531  &     Fe I  & 5166.28 &    0.00  &   -4.12  & 59.03 & 1.43 & 5.40 & 10 \\
 J20313531  &     Fe I  & 5171.60 &    1.49  &   -1.72  & 87.65 & 1.22 & 5.29 & 10 \\
 J20313531  &     Fe I  & 5191.45 &    3.04  &   -0.55  & 61.72 & 1.44 & 5.21 & 10 \\
 J20313531  &     Fe I  & 5192.34 &    3.00  &   -0.42  & 65.44 & 1.38 & 5.11 & 10 \\
 J20313531  &     Fe I  & 5194.94 &    1.56  &   -2.02  & 71.87 & 1.32 & 5.30 & 10 \\
 J20313531  &     Fe I  & 5198.71 &    2.22  &   -2.09  & 30.23 & 1.31 & 5.27 & 10 \\
 J20313531  &     Fe I  & 5202.34 &    2.18  &   -1.87  & 52.35 & 1.47 & 5.43 & 10 \\
 J20313531  &     Fe I  & 5215.18 &    3.27  &   -0.86  & 31.17 & 1.31 & 5.19 & 9 \\
 J20313531  &     Fe I  & 5216.27 &    1.61  &   -2.08  & 68.19 & 1.26 & 5.33 & 10 \\
 J20313531  &     Fe I  & 5217.39 &    3.21  &   -1.07  & 27.93 & 1.31 & 5.27 & 9 \\
 J20313531  &     Fe I  & 5225.53 &    0.11  &   -4.76  & 20.46 & 1.26 & 5.38 & 10 \\
 J20313531  &     Fe I  & 5232.94 &    2.94  &   -0.06  & 84.22 & 1.25 & 5.06 & 10 \\
 J20313531  &     Fe I  & 5242.49 &    3.63  &   -0.83  & 16.97 & 1.33 & 5.20 & 11 \\
 J20313531  &     Fe I  & 5263.31 &    3.27  &   -0.87  & 27.50 & 1.07 & 5.12 & 9 \\
 J20313531  &     Fe I  & 5266.56 &    3.00  &   -0.38  & 66.73 & 1.29 & 5.09 & 10 \\
 J20313531  &     Fe I  & 5281.79 &    3.04  &   -0.83  & 48.43 & 1.14 & 5.24 & 10 \\
 J20313531  &     Fe I  & 5283.62 &    3.24  &   -0.45  & 51.89 & 1.17 & 5.14 & 9 \\
 J20313531  &     Fe I  & 5307.36 &    1.61  &   -2.91  & 23.78 & 1.20 & 5.27 & 10 \\
 J20313531  &     Fe I  & 5324.18 &    3.21  &   -0.11  & 69.52 & 1.18 & 5.10 & 12 \\
 J20313531  &     Fe I  & 5332.90 &    1.56  &   -2.78  & 30.40 & 1.28 & 5.23 & 10 \\
 J20313531  &     Fe I  & 5339.93 &    3.27  &   -0.63  & 42.27 & 1.19 & 5.17 & 9 \\
 J20313531  &     Fe I  & 5341.02 &    1.61  &   -1.95  & 77.34 & 1.16 & 5.39 & 10 \\
 J20313531  &     Fe I  & 5364.87 &    4.45  &    0.23  & 22.59 & 1.34 & 5.16 & 10 \\
 J20313531  &     Fe I  & 5367.47 &    4.42  &    0.44  & 26.90 & 1.05 & 5.02 & 10 \\
 J20313531  &     Fe I  & 5369.96 &    4.37  &    0.54  & 35.70 & 1.19 & 5.06 & 10 \\
 J20313531  &     Fe I  & 5371.49 &    0.96  &   -1.64  & 121.90 & 1.15 & 5.37 & 10 \\
 J20313531  &     Fe I  & 5383.37 &    4.31  &    0.64  & 40.22 & 1.17 & 4.98 & 10 \\
 J20313531  &     Fe I  & 5397.13 &    0.92  &   -1.98  & 110.19 & 1.17 & 5.42 & 10 \\
 J20313531  &     Fe I  & 5405.77 &    0.99  &   -1.85  & 110.29 & 1.15 & 5.37 & 10 \\
 J20313531  &     Fe I  & 5410.91 &    4.47  &    0.40  & 23.56 & 1.28 & 5.04 & 10 \\
 J20313531  &     Fe I  & 5415.20 &    4.39  &    0.64  & 37.20 & 1.22 & 5.01 & 10 \\
 J20313531  &     Fe I  & 5429.70 &    0.96  &   -1.88  & 114.23 & 1.19 & 5.44 & 10 \\
 J20313531  &     Fe I  & 5434.52 &    1.01  &   -2.13  & 98.72 & 1.10 & 5.40 & 10 \\
 J20313531  &     Fe I  & 5497.52 &    1.01  &   -2.82  & 71.29 & 1.14 & 5.45 & 10 \\
 J20313531  &     Fe I  & 5501.47 &    0.96  &   -3.05  & 62.06 & 1.09 & 5.43 & 10 \\
 J20313531  &     Fe I  & 5506.78 &    0.99  &   -2.79  & 73.39 & 1.08 & 5.44 & 10 \\
 J20313531  &     Fe I  & 5569.62 &    3.42  &   -0.52  & 40.67 & 1.08 & 5.18 & 9 \\
 J20313531  &     Fe I  & 5586.76 &    3.37  &   -0.11  & 62.33 & 1.08 & 5.12 & 9 \\
 J20313531  &     Fe I  & 5624.54 &    3.42  &   -0.76  & 27.69 & 0.98 & 5.16 & 9 \\
 J20313531  &     Fe I  & 6065.48 &    2.61  &   -1.41  & 39.74 & 0.85 & 5.16 & 10 \\
 J20313531  &     Fe I  & 6136.61 &    2.45  &   -1.41  & 57.01 & 1.01 & 5.31 & 10 \\
 J20313531  &     Fe I  & 6137.69 &    2.59  &   -1.35  & 48.41 & 0.89 & 5.24 & 10 \\
 J20313531  &     Fe I  & 6213.43 &    2.22  &   -2.48  & 17.98 & 1.02 & 5.30 & 10 \\
 J20313531  &     Fe I  & 6219.28 &    2.20  &   -2.45  & 21.62 & 0.91 & 5.36 & 10 \\
 J20313531  &     Fe I  & 6230.72 &    2.56  &   -1.28  & 60.38 & 0.99 & 5.36 & 10 \\
 J20313531  &     Fe I  & 6246.32 &    3.60  &   -0.77  & 23.57 & 0.99 & 5.25 & 9 \\
 J20313531  &     Fe I  & 6252.56 &    2.40  &   -1.77  & 50.82 & 0.98 & 5.49 & 10 \\
 J20313531  &     Fe I  & 6265.13 &    2.18  &   -2.54  & 19.63 & 0.91 & 5.37 & 10 \\
 J20313531  &     Fe I  & 6336.82 &    3.69  &   -0.85  & 16.42 & 1.10 & 5.22 & 9 \\
 J20313531  &     Fe I  & 6393.60 &    2.43  &   -1.58  & 53.16 & 0.83 & 5.37 & 10 \\
 J20313531  &     Fe I  & 6408.02 &    3.69  &   -0.99  & 12.16 & 0.77 & 5.21 & 9 \\
 J20313531  &     Fe I  & 6411.65 &    3.65  &   -0.59  & 24.86 & 0.92 & 5.14 & 9 \\
 J20313531  &     Fe I  & 6421.35 &    2.28  &   -2.01  & 39.22 & 0.91 & 5.37 & 10 \\
 J20313531  &     Fe I  & 6430.85 &    2.18  &   -1.95  & 45.08 & 0.86 & 5.31 & 10 \\
 J20313531  &     Fe I  & 6494.98 &    2.40  &   -1.24  & 66.16 & 0.87 & 5.24 & 10 \\
 J20313531  &     Fe I  & 6592.91 &    2.73  &   -1.47  & 33.97 & 0.90 & 5.22 & 10 \\
 J20313531  &     Fe I  & 6593.87 &    2.43  &   -2.37  & 17.36 & 1.07 & 5.39 & 10 \\
 J20313531  &     Fe I  & 6677.99 &    2.69  &   -1.42  & 47.52 & 0.87 & 5.38 & 10 \\
 J20313531  &     Fe I  & 7495.07 &    4.22  &   -0.10  & 21.40 & 0.94 & 5.15 & 12 \\
 J20313531  &     Fe I  & 7511.02 &    4.18  &    0.12  & 33.93 & 1.04 & 5.17 & 9 \\
 J20313531  &    Fe II  & 4178.86 &    2.58  &   -2.51  & 47.54 & 0.89 & 5.18 & 13 \\
 J20313531  &    Fe II  & 4416.82 &    2.78  &   -2.57  & 36.31 & 0.70 & 5.21 & 14 \\
 J20313531  &    Fe II  & 4491.41 &    2.86  &   -2.71  & 21.74 & 0.77 & 5.11 & 13 \\
 J20313531  &    Fe II  & 4508.28 &    2.86  &   -2.42  & 43.06 & 0.69 & 5.28 & 14 \\
 J20313531  &    Fe II  & 4515.34 &    2.84  &   -2.60  & 36.81 & 0.79 & 5.31 & 13 \\
 J20313531  &    Fe II  & 4583.83 &    2.81  &   -1.94  & 69.71 & 0.69 & 5.27 & 14 \\
 J20313531  &    Fe II  & 4620.52 &    2.83  &   -3.21  & 10.81 & 0.73 & 5.20 & 13 \\
 J20313531  &    Fe II  & 5197.58 &    3.23  &   -2.22  & 32.26 & 1.31 & 5.22 & 13 \\
 J20313531  &    Fe II  & 5234.63 &    3.22  &   -2.18  & 39.71 & 1.62 & 5.32 & 13 \\
 J20313531  &    Fe II  & 5276.00 &    3.20  &   -2.01  & 48.87 & 1.29 & 5.29 & 13 \\
 J20313531  &     Ni I  & 3472.54 &    0.11  &   -0.79  & 107.15 & 3.50 & 3.66 & 15 \\
 J20313531  &     Ni I  & 3500.85 &    0.17  &   -1.27  & 101.86 & 2.58 & 4.04 & 15 \\
 J20313531  &     Ni I  & 3597.70 &    0.21  &   -1.10  & 105.95 & 2.15 & 3.94 & 15 \\
 J20313531  &     Ni I  & 3807.14 &    0.42  &   -1.23  & 91.81 & 1.28 & 3.77 & 15 \\
 J20313531  &     Ni I  & 4470.48 &    3.40  &   -0.30  & 8.79 & 0.74 & 3.82 & 15 \\
 J20313531  &     Ni I  & 4604.99 &    3.48  &   -0.24  & 13.52 & 1.04 & 4.05 & 15 \\
 J20313531  &     Ni I  & 4648.65 &    3.42  &   -0.09  & 13.70 & 0.68 & 3.84 & 15 \\
 J20313531  &     Ni I  & 4714.42 &    3.38  &    0.25  & 28.73 & 0.72 & 3.87 & 15 \\
 J20313531  &     Ni I  & 4756.52 &    3.48  &   -0.27  & 9.71 & 0.79 & 3.91 & 15 \\
 J20313531  &     Ni I  & 4904.41 &    3.54  &   -0.17  & 12.24 & 0.73 & 3.98 & 1 \\
 J20313531  &     Ni I  & 5017.58 &    3.54  &   -0.03  & 12.46 & 0.95 & 3.84 & 15 \\
 J20313531  &     Ni I  & 5476.90 &    1.83  &   -0.78  & 72.92 & 1.37 & 4.07 & 15 \\
 J20313531  &     Ni I  & 6643.63 &    1.68  &   -2.22  & 14.03 & 0.96 & 4.00 & 15 \\
 J20313531  &     Ni I  & 6767.77 &    1.83  &   -2.14  & 14.08 & 0.99 & 4.08 & 15 \\
 J20313531  &     Zn I  & 4722.16 &    4.03  &   -0.37  & 15.16 & 0.72 & 2.50 & 16 \\
 J20313531  &     Zn I  & 4810.54 &    4.08  &   -0.15  & 20.82 & 0.80 & 2.50 & 16 \\
 J20313531  &    C-H I  & 4312.00 &     NaN  &     NaN  &     synth  &    synth  & 6.46 & NaN \\
 J20313531  &    C-H I  & 4323.00 &     NaN  &     NaN  &     synth  &    synth  & 6.42 & NaN \\
 J20313531  &    C-H I  & 4230.00 &     NaN  &     NaN  &     synth  &    synth  & 6.42 & NaN \\
 J20313531  &    C-H I  & 4311.00 &     NaN  &     NaN  &     synth  &    synth  & 6.41 & NaN \\
 J20313531  &     Li I  & 6707.80 &    0.00  &    0.17  &     synth  &    synth  & 1.16 & 17 \\
 J20313531  &    Sc II  & 3572.53 &    0.02  &    0.27  &     synth  &    synth  & 0.81 & 18 \\
 J20313531  &    Sc II  & 3590.47 &    0.02  &   -0.55  &     synth  &    synth  & 0.85 & 18 \\
 J20313531  &    Sc II  & 4246.82 &    0.32  &    0.24  &     synth  &    synth  & 0.91 & 18 \\
 J20313531  &    Sc II  & 4324.99 &    0.60  &   -0.44  &     synth  &    synth  & 0.89 & NaN \\
 J20313531  &    Sc II  & 4374.47 &    0.62  &   -0.46  &     synth  &    synth  & 0.98 & NaN \\
 J20313531  &    Sc II  & 4400.39 &    0.61  &   -0.54  &     synth  &    synth  & 0.98 & NaN \\
 J20313531  &    Sc II  & 4415.56 &    0.60  &   -0.68  &     synth  &    synth  & 1.01 & NaN \\
 J20313531  &    Sc II  & 4670.41 &    1.36  &   -0.60  &     synth  &    synth  & 0.99 & NaN \\
 J20313531  &    Sc II  & 5031.02 &    1.36  &   -0.41  &     synth  &    synth  & 0.97 & NaN \\
 J20313531  &    Sc II  & 5526.79 &    1.77  &   -0.01  &     synth  &    synth  & 0.86 & NaN \\
 J20313531  &    Sc II  & 5657.90 &    1.51  &   -0.54  &     synth  &    synth  & 0.97 & NaN \\
 J20313531  &      V I  & 4111.78 &    0.30  &    0.40  &     synth  &    synth  & 1.57 & 19 \\
 J20313531  &      V I  & 4379.23 &    0.30  &    0.58  &     synth  &    synth  & 1.61 & 19 \\
 J20313531  &      V I  & 4389.98 &    0.28  &    0.22  &     synth  &    synth  & 1.53 & 19 \\
 J20313531  &     V II  & 3517.30 &    1.13  &   -0.24  &     synth  &    synth  & 1.86 & 20 \\
 J20313531  &     V II  & 3530.77 &    1.07  &   -0.53  &     synth  &    synth  & 1.72 & 20 \\
 J20313531  &     V II  & 3545.20 &    1.09  &   -0.32  &     synth  &    synth  & 1.68 & 20 \\
 J20313531  &     V II  & 3715.46 &    1.57  &   -0.22  &     synth  &    synth  & 1.72 & 20 \\
 J20313531  &     V II  & 3727.34 &    1.69  &   -0.23  &     synth  &    synth  & 1.74 & 20 \\
 J20313531  &     V II  & 3951.96 &    1.48  &   -0.73  &     synth  &    synth  & 1.86 & 20 \\
 J20313531  &     V II  & 4002.93 &    1.43  &   -1.44  &     synth  &    synth  & 1.86 & 20 \\
 J20313531  &     V II  & 4002.93 &    1.43  &   -1.44  &     synth  &    synth  & 1.85 & 20 \\
 J20313531  &     Mn I  & 4030.75 &    0.00  &   -0.50  &     synth  &    synth  & 2.91 & 21 \\
 J20313531  &     Mn I  & 4033.06 &    0.00  &   -0.65  &     synth  &    synth  & 2.87 & 21 \\
 J20313531  &     Mn I  & 4034.48 &    0.00  &   -0.84  &     synth  &    synth  & 2.77 & 21 \\
 J20313531  &     Mn I  & 4041.35 &    2.11  &    0.28  &     synth  &    synth  & 2.70 & 21 \\
 J20313531  &     Mn I  & 4754.04 &    2.28  &   -0.08  &     synth  &    synth  & 2.57 & 21 \\
 J20313531  &     Mn I  & 4762.37 &    2.89  &    0.30  &     synth  &    synth  & 2.32 & 21 \\
 J20313531  &     Mn I  & 4823.52 &    2.32  &    0.14  &     synth  &    synth  & 2.60 & 21 \\
 J20313531  &    Mn II  & 3441.99 &    1.78  &   -0.35  &     synth  &    synth  & 2.77 & 21 \\
 J20313531  &    Mn II  & 3460.32 &    1.81  &   -0.63  &     synth  &    synth  & 2.74 & 21 \\
 J20313531  &    Mn II  & 3482.90 &    1.83  &   -0.84  &     synth  &    synth  & 3.17 & 21 \\
 J20313531  &    Mn II  & 3488.68 &    1.85  &   -0.94  &     synth  &    synth  & 3.04 & 21 \\
 J20313531  &    Mn II  & 3497.53 &    1.85  &   -1.42  &     synth  &    synth  & 2.89 & 21 \\
 J20313531  &     Co I  & 3433.04 &    0.63  &   -0.18  &     synth  &    synth  & 2.73 & 22 \\
 J20313531  &     Co I  & 3455.24 &    0.22  &   -1.19  &     synth  &    synth  & 2.94 & 22 \\
 J20313531  &     Co I  & 3489.40 &    0.92  &    0.18  &     synth  &    synth  & 2.68 & 22 \\
 J20313531  &     Co I  & 3491.32 &    0.22  &   -1.41  &     synth  &    synth  & 3.04 & 22 \\
 J20313531  &     Co I  & 3502.28 &    0.43  &    0.11  &     synth  &    synth  & 2.91 & 22 \\
 J20313531  &     Co I  & 3502.28 &    0.43  &    0.11  &     synth  &    synth  & 2.99 & 22 \\
 J20313531  &     Co I  & 3518.34 &    1.05  &    0.00  &     synth  &    synth  & 2.63 & 22 \\
 J20313531  &     Co I  & 3521.57 &    0.43  &   -0.74  &     synth  &    synth  & 2.72 & 22 \\
 J20313531  &     Co I  & 3529.03 &    0.17  &   -0.89  &     synth  &    synth  & 2.69 & 22 \\
 J20313531  &     Co I  & 3529.03 &    0.17  &   -0.89  &     synth  &    synth  & 2.58 & 22 \\
 J20313531  &     Co I  & 3550.59 &    0.17  &   -1.59  &     synth  &    synth  & 2.92 & 22 \\
 J20313531  &     Co I  & 3842.05 &    0.92  &   -0.74  &     synth  &    synth  & 2.92 & 22 \\
 J20313531  &     Co I  & 3845.47 &    0.92  &    0.06  &     synth  &    synth  & 2.81 & 22 \\
 J20313531  &     Co I  & 3894.08 &    1.05  &    0.12  &     synth  &    synth  & 2.63 & 22 \\
 J20313531  &     Co I  & 3995.31 &    0.92  &   -0.18  &     synth  &    synth  & 2.70 & 22 \\
 J20313531  &     Co I  & 4118.77 &    1.05  &   -0.48  &     synth  &    synth  & 2.83 & 22 \\
 J20313531  &     Co I  & 4121.32 &    0.92  &   -0.33  &     synth  &    synth  & 2.90 & 22 \\
 J20313531  &    Sr II  & 4077.71 &    0.00  &    0.15  &     synth  &    synth  & 0.72 & 23 \\
 J20313531  &    Sr II  & 4215.52 &    0.00  &   -0.17  &     synth  &    synth  & 0.69 & 23 \\
 J20313531  &     Y II  & 3549.00 &    0.13  &   -0.29  &     synth  &    synth  & -0.17 & 24 \\
 J20313531  &     Y II  & 3600.73 &    0.18  &     0.34  &     synth  &    synth  & -0.41 & 24 \\
 J20313531  &     Y II  & 3601.92 &    0.10  &   -0.15  &     synth  &    synth  & -0.39 & 24 \\
 J20313531  &     Y II  & 3611.04 &    0.13  &    0.05  &     synth  &    synth  & -0.21 & 24 \\
 J20313531  &     Y II  & 3710.29 &    0.18  &    0.51  &     synth  &    synth  & -0.35 & 24 \\
 J20313531  &     Y II  & 3774.33 &    0.13  &    0.29  &     synth  &    synth  & -0.23 & NaN \\
 J20313531  &     Y II  & 3832.89 &    0.18  &   -0.34  &     synth  &    synth  & -0.31 & 24 \\
 J20313531  &     Y II  & 3982.59 &    0.13  &   -0.56  &     synth  &    synth  & -0.18 & 24 \\
 J20313531  &     Y II  & 4398.01 &    0.13  &   -0.75  &     synth  &    synth  & -0.48 & 24 \\
 J20313531  &     Y II  & 4883.68 &    1.08  &    0.19  &     synth  &    synth  & -0.50 & 24 \\
 J20313531  &     Y II  & 4900.12 &    1.03  &    0.03  &     synth  &    synth  & -0.50 & 24 \\
 J20313531  &     Y II  & 5205.72 &    1.03  &    -0.28  &     synth  &    synth  & -0.47 & 24 \\
 J20313531  &    Zr II  & 3430.53 &    0.47  &    -0.16  &     synth  &    synth  & 0.54 & 25 \\
 J20313531  &    Zr II  & 3479.02 &    0.53  &   -0.67  &     synth  &    synth  & 0.33 & 25 \\
 J20313531  &    Zr II  & 3505.67 &     0.16  &     -0.39  &     synth  &    synth  & 0.53 & 25 \\
 J20313531  &    Zr II  & 3551.95 &     0.10  &     -0.36  &     synth  &    synth  & 0.54 & 25 \\
 J20313531  &    Zr II  & 3998.96 &    0.56  &   -0.52  &     synth  &    synth  & 0.57 & 25 \\
 J20313531  &    Zr II  & 4149.20 &    0.80  &   -0.04  &     synth  &    synth  & 0.52 & 25 \\
 J20313531  &    Zr II  & 4161.20 &     0.71  &     -0.59  &     synth  &    synth  & 0.55 & 25 \\
 J20313531  &    Zr II  & 4208.98 &     0.71  &     -0.51  &     synth  &    synth  & 0.56 & 25 \\
 J20313531  &    Zr II  & 4211.88 &     0.53  &     -1.04  &     synth  &    synth  & 0.57 & 25 \\
 J20313531  &    Ba II  & 4554.03 &    0.00  &    0.14  &     synth  &    synth  & -0.44 & 26 \\
 J20313531  &    Ba II  & 4934.08 &    0.00  &   -0.16  &     synth  &    synth  & -0.47 & 26 \\
 J20313531  &    Ba II  & 5853.68 &    0.60  &   -0.91  &     synth  &    synth  & -0.41 & 26 \\
 J20313531  &    Ba II  & 6141.71 &    0.70  &   -0.03  &     synth  &    synth  & -0.54 & 26 \\
 J20313531  &    Ba II  & 6496.90 &    0.60  &   -0.41  &     synth  &    synth  & -0.36 & 26 \\
 J20313531  &    La II  & 3949.10 &    0.40  &    0.49  &     synth  &    synth  & -1.35 & 27 \\
 J20313531  &    La II  & 4077.34 &    0.24  &   -0.06  &     synth  &    synth  & -1.03 & 27 \\
 J20313531  &    Nd II  & 3991.74 &    0.00  &    -0.26  &     synth  &    synth  & -0.76 & 28 \\
 J20313531  &    Nd II  & 4303.57 &    0.00  &    0.08  &     synth  &    synth  & -0.50 & 28 \\
 J20313531  &    Eu II  & 3819.67 &    0.00  &    0.51  &     synth  &    synth  & -1.57 & 29 \\
 J20313531  &    Eu II  & 4129.72 &    0.00  &    0.22  &     synth  &    synth  & -1.43 & 29 \\
 J20313531  &    Eu II  & 4205.04 &    0.00  &    0.21  &     synth  &    synth  & -1.49 & 29 \\
 J20313531  &    Dy II  & 3944.68 &    0.00  &    0.11  &     synth  &    synth  & -0.98 & 30 \\
 J20313531  &    Dy II  & 4077.97 &    0.10  &    -0.04  &     synth  &    synth  & -0.90 & 30 \\
 J20313531  &    Er II  & 3499.10 &    0.06  &    0.29  &     synth  &    synth  & -1.04 & 31 \\
 J20313531  &    Er II  & 3906.31 &    0.00  &    0.12  &     synth  &    synth  & -0.97 & 31 \\
 J20313531  &    Yb II  & 3694.19 &    0.00  &   -0.30  &     synth  &    synth  & -1.20 & 32 \\
 J20313531  &     Al I  & 3944.00 &    0.00  &   -0.64  &     synth  &    synth  & 3.28 & 1 \\
 J20313531  &     Al I  & 3961.52 &    0.01  &   -0.33  &     synth  &    synth  & 3.24 & 1 \\
 J21402305  &      O I  & 7771.94 &    9.15  &    0.37  & 10.92 & 0.53 & 7.27 & 1 \\
 J21402305  &      O I  & 7774.17 &    9.15  &    0.22  & 3.32 & 0.30 & 6.81 & 1 \\
 J21402305  &      O I  & 7775.39 &    9.15  &    0.00  & 2.58 & 0.42 & 6.92 & 1 \\
 J21402305  &     Na I  & 5889.95 &    0.00  &    0.11  & 175.04 & 0.38 & 4.00 & 1 \\
 J21402305  &     Na I  & 5895.92 &    0.00  &   -0.19  & 155.24 & 0.36 & 3.99 & 1 \\
 J21402305  &     Mg I  & 3829.35 &    2.71  &   -0.23  & 159.88 & 0.62 & 5.05 & 1 \\
 J21402305  &     Mg I  & 3832.30 &    2.71  &    0.25  & 193.63 & 0.77 & 4.94 & 1 \\
 J21402305  &     Mg I  & 4167.27 &    4.35  &   -0.74  & 41.29 & 1.07 & 5.16 & 1 \\
 J21402305  &     Mg I  & 4702.99 &    4.33  &   -0.44  & 59.66 & 0.34 & 5.08 & 1 \\
 J21402305  &     Mg I  & 5172.68 &    2.71  &   -0.36  & 181.91 & 0.59 & 5.11 & 2 \\
 J21402305  &     Mg I  & 5183.60 &    2.72  &   -0.17  & 203.17 & 0.57 & 5.15 & 2 \\
 J21402305  &     Mg I  & 5528.40 &    4.35  &   -0.55  & 63.25 & 0.44 & 5.24 & 2 \\
 J21402305  &     Mg I  & 5711.09 &    4.35  &   -1.84  & 6.61 & 0.45 & 5.23 & 2 \\
 J21402305  &     Si I  & 3905.52 &    1.91  &   -1.04  & 204.72 & 0.75 & 5.26 & 1 \\
 J21402305  &     Si I  & 5708.40 &    4.95  &   -1.47  & 4.59 & 0.51 & 5.29 & 1 \\
 J21402305  &      K I  & 7698.96 &    0.00  &   -0.18  & 19.34 & 0.39 & 2.52 & 1 \\
 J21402305  &     Ca I  & 4226.74 &    0.00  &    0.24  & 162.31 & 0.82 & 3.33 & 3 \\
 J21402305  &     Ca I  & 4283.01 &    1.89  &   -0.20  & 43.21 & 0.67 & 3.67 & 3 \\
 J21402305  &     Ca I  & 4318.65 &    1.90  &   -0.21  & 33.93 & 0.38 & 3.52 & 1 \\
 J21402305  &     Ca I  & 4425.44 &    1.88  &   -0.41  & 27.96 & 0.35 & 3.57 & 3 \\
 J21402305  &     Ca I  & 4435.69 &    1.89  &   -0.55  & 25.37 & 0.41 & 3.66 & 3 \\
 J21402305  &     Ca I  & 4454.78 &    1.90  &    0.26  & 64.64 & 0.34 & 3.57 & 1 \\
 J21402305  &     Ca I  & 4455.89 &    1.90  &   -0.55  & 23.77 & 0.34 & 3.64 & 3 \\
 J21402305  &     Ca I  & 5588.76 &    2.52  &    0.30  & 30.38 & 0.42 & 3.58 & 3 \\
 J21402305  &     Ca I  & 5601.29 &    2.53  &   -0.57  & 7.12 & 0.50 & 3.71 & 3 \\
 J21402305  &     Ca I  & 5857.45 &    2.93  &    0.17  & 14.33 & 1.09 & 3.76 & 3 \\
 J21402305  &     Ca I  & 6102.72 &    1.88  &   -0.81  & 20.53 & 0.40 & 3.72 & 3 \\
 J21402305  &     Ca I  & 6122.22 &    1.89  &   -0.33  & 43.50 & 0.41 & 3.71 & 3 \\
 J21402305  &     Ca I  & 6162.17 &    1.90  &   -0.11  & 58.06 & 0.38 & 3.73 & 3 \\
 J21402305  &     Ca I  & 6169.56 &    2.53  &   -0.60  & 7.14 & 0.37 & 3.73 & 3 \\
 J21402305  &     Ca I  & 6439.07 &    2.52  &    0.33  & 38.55 & 0.38 & 3.67 & 3 \\
 J21402305  &     Ca I  & 6449.81 &    2.52  &   -0.55  & 9.84 & 0.48 & 3.81 & 3 \\
 J21402305  &     Ti I  & 3989.76 &    0.02  &   -0.13  & 55.52 & 0.49 & 2.24 & 4 \\
 J21402305  &     Ti I  & 3998.64 &    0.05  &    0.02  & 59.55 & 0.49 & 2.20 & 4 \\
 J21402305  &     Ti I  & 4512.73 &    0.84  &   -0.40  & 8.22 & 0.32 & 2.29 & 4 \\
 J21402305  &     Ti I  & 4518.02 &    0.83  &   -0.25  & 13.94 & 0.36 & 2.38 & 4 \\
 J21402305  &     Ti I  & 4533.24 &    0.85  &    0.54  & 39.90 & 0.33 & 2.21 & 4 \\
 J21402305  &     Ti I  & 4534.78 &    0.84  &    0.35  & 31.88 & 0.35 & 2.25 & 4 \\
 J21402305  &     Ti I  & 4548.76 &    0.83  &   -0.28  & 10.38 & 0.35 & 2.27 & 4 \\
 J21402305  &     Ti I  & 4555.48 &    0.85  &   -0.40  & 8.06 & 0.35 & 2.29 & 4 \\
 J21402305  &     Ti I  & 4656.47 &    0.00  &   -1.28  & 12.01 & 0.33 & 2.36 & 1 \\
 J21402305  &     Ti I  & 4681.91 &    0.05  &   -1.01  & 19.82 & 0.37 & 2.40 & 1 \\
 J21402305  &     Ti I  & 4840.87 &    0.90  &   -0.43  & 6.50 & 0.35 & 2.25 & 4 \\
 J21402305  &     Ti I  & 4981.73 &    0.84  &    0.57  & 47.24 & 0.42 & 2.26 & 4 \\
 J21402305  &     Ti I  & 4991.07 &    0.84  &    0.45  & 42.69 & 0.82 & 2.30 & 4 \\
 J21402305  &     Ti I  & 4999.50 &    0.83  &    0.32  & 35.53 & 0.43 & 2.29 & 4 \\
 J21402305  &     Ti I  & 5016.16 &    0.85  &   -0.48  & 7.18 & 0.44 & 2.28 & 4 \\
 J21402305  &     Ti I  & 5064.65 &    0.05  &   -0.94  & 22.38 & 0.54 & 2.37 & 4 \\
 J21402305  &     Ti I  & 5173.74 &    0.00  &   -1.06  & 17.34 & 0.55 & 2.29 & 4 \\
 J21402305  &     Ti I  & 5192.97 &    0.02  &   -0.95  & 24.67 & 0.51 & 2.39 & 4 \\
 J21402305  &     Ti I  & 5210.38 &    0.05  &   -0.82  & 25.61 & 0.54 & 2.31 & 4 \\
 J21402305  &    Ti II  & 3759.29 &    0.61  &    0.28  & 173.84 & 0.71 & 2.69 & 5 \\
 J21402305  &    Ti II  & 3761.32 &    0.57  &    0.18  & 169.88 & 0.72 & 2.67 & 5 \\
 J21402305  &    Ti II  & 4028.34 &    1.89  &   -0.92  & 41.08 & 0.44 & 2.20 & 5 \\
 J21402305  &    Ti II  & 4337.91 &    1.08  &   -0.96  & 95.93 & 0.37 & 2.29 & 6 \\
 J21402305  &    Ti II  & 4394.06 &    1.22  &   -1.77  & 49.85 & 0.37 & 2.38 & 5 \\
 J21402305  &    Ti II  & 4395.03 &    1.08  &   -0.54  & 115.63 & 0.36 & 2.34 & 5 \\
 J21402305  &    Ti II  & 4395.84 &    1.24  &   -1.93  & 36.03 & 0.36 & 2.33 & 5 \\
 J21402305  &    Ti II  & 4399.77 &    1.24  &   -1.20  & 79.59 & 0.34 & 2.36 & 5 \\
 J21402305  &    Ti II  & 4409.52 &    1.23  &   -2.53  & 12.92 & 0.34 & 2.35 & 5 \\
 J21402305  &    Ti II  & 4417.71 &    1.17  &   -1.19  & 84.82 & 0.33 & 2.37 & 6 \\
 J21402305  &    Ti II  & 4418.33 &    1.24  &   -1.99  & 37.15 & 0.35 & 2.41 & 5 \\
 J21402305  &    Ti II  & 4443.80 &    1.08  &   -0.71  & 108.05 & 0.35 & 2.31 & 5 \\
 J21402305  &    Ti II  & 4444.55 &    1.12  &   -2.20  & 36.74 & 0.37 & 2.47 & 5 \\
 J21402305  &    Ti II  & 4450.48 &    1.08  &   -1.52  & 74.68 & 0.36 & 2.38 & 5 \\
 J21402305  &    Ti II  & 4464.45 &    1.16  &   -1.81  & 52.74 & 0.32 & 2.39 & 6 \\
 J21402305  &    Ti II  & 4470.85 &    1.17  &   -2.02  & 35.22 & 0.34 & 2.31 & 6 \\
 J21402305  &    Ti II  & 4493.52 &    1.08  &   -2.78  & 10.58 & 0.37 & 2.32 & 5 \\
 J21402305  &    Ti II  & 4501.27 &    1.12  &   -0.77  & 108.27 & 0.37 & 2.40 & 5 \\
 J21402305  &    Ti II  & 4533.96 &    1.24  &   -0.53  & 111.90 & 0.37 & 2.37 & 6 \\
 J21402305  &    Ti II  & 4571.97 &    1.57  &   -0.31  & 100.86 & 0.33 & 2.29 & 5 \\
 J21402305  &    Ti II  & 4583.41 &    1.16  &   -2.84  & 12.76 & 0.36 & 2.56 & 5 \\
 J21402305  &    Ti II  & 4657.20 &    1.24  &   -2.29  & 23.25 & 0.41 & 2.40 & 5 \\
 J21402305  &    Ti II  & 4708.66 &    1.24  &   -2.35  & 23.14 & 0.32 & 2.46 & 5 \\
 J21402305  &    Ti II  & 4798.53 &    1.08  &   -2.66  & 19.06 & 0.38 & 2.47 & 5 \\
 J21402305  &    Ti II  & 5129.16 &    1.89  &   -1.34  & 33.62 & 0.65 & 2.40 & 5 \\
 J21402305  &    Ti II  & 5185.90 &    1.89  &   -1.41  & 24.60 & 0.57 & 2.28 & 5 \\
 J21402305  &    Ti II  & 5188.69 &    1.58  &   -1.05  & 71.61 & 0.57 & 2.35 & 6 \\
 J21402305  &    Ti II  & 5336.79 &    1.58  &   -1.60  & 39.37 & 0.50 & 2.38 & 5 \\
 J21402305  &    Ti II  & 5381.02 &    1.57  &   -1.97  & 24.12 & 0.52 & 2.44 & 5 \\
 J21402305  &    Ti II  & 5418.77 &    1.58  &   -2.13  & 17.21 & 0.52 & 2.43 & 5 \\
 J21402305  &     Cr I  & 3578.68 &    0.00  &    0.42  & 111.62 & 1.24 & 2.50 & 7 \\
 J21402305  &     Cr I  & 4274.80 &    0.00  &   -0.22  & 112.46 & 0.40 & 2.73 & 7 \\
 J21402305  &     Cr I  & 4289.72 &    0.00  &   -0.37  & 103.09 & 0.39 & 2.63 & 7 \\
 J21402305  &     Cr I  & 4545.95 &    0.94  &   -1.37  & 14.54 & 0.36 & 2.83 & 7 \\
 J21402305  &     Cr I  & 4646.15 &    1.03  &   -0.74  & 35.69 & 0.33 & 2.81 & 7 \\
 J21402305  &     Cr I  & 4651.28 &    0.98  &   -1.46  & 13.07 & 0.35 & 2.91 & 7 \\
 J21402305  &     Cr I  & 5296.69 &    0.98  &   -1.36  & 17.33 & 0.51 & 2.91 & 7 \\
 J21402305  &     Cr I  & 5298.28 &    0.98  &   -1.14  & 26.18 & 0.53 & 2.91 & 7 \\
 J21402305  &     Cr I  & 5345.80 &    1.00  &   -0.95  & 28.34 & 0.50 & 2.79 & 7 \\
 J21402305  &     Cr I  & 5348.31 &    1.00  &   -1.21  & 17.32 & 0.46 & 2.78 & 7 \\
 J21402305  &     Cr I  & 5409.77 &    1.03  &   -0.67  & 40.41 & 0.52 & 2.77 & 7 \\
 J21402305  &    Cr II  & 4558.64 &    4.07  &   -0.43  & 25.08 & 0.37 & 2.96 & 8 \\
 J21402305  &    Cr II  & 4588.20 &    4.07  &   -0.65  & 16.02 & 0.33 & 2.93 & 8 \\
 J21402305  &    Cr II  & 4618.81 &    4.07  &   -0.89  & 11.80 & 0.37 & 3.01 & 8 \\
 J21402305  &     Fe I  & 3450.33 &    2.22  &   -0.90  & 59.60 & 1.90 & 4.52 & 10 \\
 J21402305  &     Fe I  & 3618.77 &    0.99  &   -0.00  & 154.84 & 1.34 & 4.42 & 10 \\
 J21402305  &     Fe I  & 3765.54 &    3.24  &    0.48  & 60.33 & 0.73 & 4.16 & 10 \\
 J21402305  &     Fe I  & 3786.68 &    1.01  &   -2.18  & 70.23 & 0.61 & 4.45 & 10 \\
 J21402305  &     Fe I  & 3787.88 &    1.01  &   -0.84  & 119.09 & 0.60 & 4.38 & 10 \\
 J21402305  &     Fe I  & 3808.73 &    2.56  &   -1.17  & 28.28 & 0.68 & 4.42 & 11 \\
 J21402305  &     Fe I  & 3841.05 &    1.61  &   -0.04  & 117.92 & 0.63 & 4.20 & 10 \\
 J21402305  &     Fe I  & 3865.52 &    1.01  &   -0.95  & 116.66 & 0.55 & 4.36 & 10 \\
 J21402305  &     Fe I  & 3899.71 &    0.09  &   -1.52  & 136.69 & 0.50 & 4.46 & 10 \\
 J21402305  &     Fe I  & 3902.95 &    1.56  &   -0.44  & 110.98 & 0.58 & 4.34 & 10 \\
 J21402305  &     Fe I  & 3922.91 &    0.05  &   -1.63  & 139.27 & 0.46 & 4.57 & 10 \\
 J21402305  &     Fe I  & 3949.95 &    2.18  &   -1.25  & 46.74 & 0.49 & 4.40 & 10 \\
 J21402305  &     Fe I  & 3977.74 &    2.20  &   -1.12  & 52.14 & 0.52 & 4.38 & 10 \\
 J21402305  &     Fe I  & 4005.24 &    1.56  &   -0.58  & 111.51 & 0.43 & 4.46 & 10 \\
 J21402305  &     Fe I  & 4067.98 &    3.21  &   -0.53  & 24.08 & 0.45 & 4.40 & 9 \\
 J21402305  &     Fe I  & 4114.44 &    2.83  &   -1.30  & 11.31 & 0.40 & 4.34 & 10 \\
 J21402305  &     Fe I  & 4132.06 &    1.61  &   -0.68  & 107.53 & 0.39 & 4.47 & 10 \\
 J21402305  &     Fe I  & 4143.87 &    1.56  &   -0.51  & 111.98 & 0.37 & 4.35 & 10 \\
 J21402305  &     Fe I  & 4147.67 &    1.49  &   -2.07  & 53.08 & 0.36 & 4.50 & 10 \\
 J21402305  &     Fe I  & 4156.80 &    2.83  &   -0.81  & 33.46 & 0.40 & 4.44 & 10 \\
 J21402305  &     Fe I  & 4157.78 &    3.42  &   -0.40  & 21.14 & 0.41 & 4.43 & 10 \\
 J21402305  &     Fe I  & 4181.76 &    2.83  &   -0.37  & 52.27 & 0.43 & 4.34 & 10 \\
 J21402305  &     Fe I  & 4184.89 &    2.83  &   -0.87  & 24.24 & 0.39 & 4.30 & 10 \\
 J21402305  &     Fe I  & 4187.04 &    2.45  &   -0.56  & 66.31 & 0.39 & 4.34 & 12 \\
 J21402305  &     Fe I  & 4187.80 &    2.42  &   -0.51  & 68.42 & 0.40 & 4.29 & 10 \\
 J21402305  &     Fe I  & 4195.33 &    3.33  &   -0.49  & 28.68 & 0.42 & 4.59 & 10 \\
 J21402305  &     Fe I  & 4202.03 &    1.49  &   -0.69  & 107.05 & 0.38 & 4.31 & 10 \\
 J21402305  &     Fe I  & 4222.21 &    2.45  &   -0.91  & 48.02 & 0.43 & 4.36 & 10 \\
 J21402305  &     Fe I  & 4227.43 &    3.33  &    0.27  & 63.81 & 0.44 & 4.48 & 10 \\
 J21402305  &     Fe I  & 4233.60 &    2.48  &   -0.60  & 62.39 & 0.39 & 4.33 & 12 \\
 J21402305  &     Fe I  & 4250.12 &    2.47  &   -0.38  & 72.34 & 0.36 & 4.29 & 10 \\
 J21402305  &     Fe I  & 4250.79 &    1.56  &   -0.71  & 103.29 & 0.36 & 4.30 & 10 \\
 J21402305  &     Fe I  & 4260.47 &    2.40  &    0.08  & 96.20 & 0.37 & 4.28 & 10 \\
 J21402305  &     Fe I  & 4282.40 &    2.18  &   -0.78  & 67.30 & 0.37 & 4.26 & 10 \\
 J21402305  &     Fe I  & 4415.12 &    1.61  &   -0.62  & 112.46 & 0.33 & 4.44 & 10 \\
 J21402305  &     Fe I  & 4430.61 &    2.22  &   -1.73  & 30.53 & 0.37 & 4.58 & 10 \\
 J21402305  &     Fe I  & 4442.34 &    2.20  &   -1.23  & 57.58 & 0.39 & 4.53 & 10 \\
 J21402305  &     Fe I  & 4447.72 &    2.22  &   -1.36  & 47.50 & 0.38 & 4.51 & 11 \\
 J21402305  &     Fe I  & 4461.65 &    0.09  &   -3.19  & 95.10 & 0.34 & 4.79 & 10 \\
 J21402305  &     Fe I  & 4466.55 &    2.83  &   -0.60  & 54.66 & 0.34 & 4.58 & 10 \\
 J21402305  &     Fe I  & 4489.74 &    0.12  &   -3.90  & 52.87 & 0.36 & 4.68 & 10 \\
 J21402305  &     Fe I  & 4494.56 &    2.20  &   -1.14  & 60.71 & 0.35 & 4.49 & 10 \\
 J21402305  &     Fe I  & 4531.15 &    1.48  &   -2.10  & 55.88 & 0.36 & 4.52 & 10 \\
 J21402305  &     Fe I  & 4592.65 &    1.56  &   -2.46  & 38.43 & 0.38 & 4.67 & 10 \\
 J21402305  &     Fe I  & 4602.00 &    1.61  &   -3.13  & 6.33 & 0.32 & 4.45 & 10 \\
 J21402305  &     Fe I  & 4602.94 &    1.49  &   -2.21  & 53.26 & 0.36 & 4.60 & 10 \\
 J21402305  &     Fe I  & 4647.43 &    2.95  &   -1.35  & 12.55 & 0.36 & 4.54 & 10 \\
 J21402305  &     Fe I  & 4733.59 &    1.49  &   -2.99  & 16.95 & 0.38 & 4.64 & 10 \\
 J21402305  &     Fe I  & 4736.77 &    3.21  &   -0.67  & 24.29 & 0.36 & 4.50 & 9 \\
 J21402305  &     Fe I  & 4871.32 &    2.87  &   -0.34  & 54.19 & 0.35 & 4.32 & 12 \\
 J21402305  &     Fe I  & 4872.14 &    2.88  &   -0.57  & 41.74 & 0.35 & 4.35 & 10 \\
 J21402305  &     Fe I  & 4890.76 &    2.88  &   -0.38  & 52.45 & 0.34 & 4.34 & 12 \\
 J21402305  &     Fe I  & 4891.49 &    2.85  &   -0.11  & 68.56 & 0.34 & 4.32 & 10 \\
 J21402305  &     Fe I  & 4903.31 &    2.88  &   -0.89  & 27.51 & 0.36 & 4.40 & 12 \\
 J21402305  &     Fe I  & 4918.99 &    2.86  &   -0.34  & 56.31 & 0.36 & 4.34 & 10 \\
 J21402305  &     Fe I  & 4920.50 &    2.83  &    0.07  & 76.60 & 0.36 & 4.26 & 10 \\
 J21402305  &     Fe I  & 4924.77 &    2.28  &   -2.11  & 10.35 & 0.37 & 4.42 & 10 \\
 J21402305  &     Fe I  & 4938.81 &    2.88  &   -1.08  & 21.47 & 0.38 & 4.45 & 10 \\
 J21402305  &     Fe I  & 4939.69 &    0.86  &   -3.25  & 38.25 & 0.37 & 4.61 & 10 \\
 J21402305  &     Fe I  & 4966.09 &    3.33  &   -0.79  & 14.79 & 0.38 & 4.48 & 9 \\
 J21402305  &     Fe I  & 4994.13 &    0.92  &   -2.97  & 47.61 & 0.38 & 4.55 & 10 \\
 J21402305  &     Fe I  & 5001.86 &    3.88  &   -0.01  & 15.92 & 0.43 & 4.36 & 12 \\
 J21402305  &     Fe I  & 5005.71 &    3.88  &   -0.12  & 12.46 & 0.44 & 4.35 & 12 \\
 J21402305  &     Fe I  & 5006.12 &    2.83  &   -0.62  & 42.89 & 0.41 & 4.36 & 10 \\
 J21402305  &     Fe I  & 5049.82 &    2.28  &   -1.36  & 42.25 & 0.51 & 4.45 & 10 \\
 J21402305  &     Fe I  & 5051.63 &    0.92  &   -2.76  & 67.90 & 0.46 & 4.68 & 10 \\
 J21402305  &     Fe I  & 5068.77 &    2.94  &   -1.04  & 20.77 & 0.74 & 4.45 & 10 \\
 J21402305  &     Fe I  & 5083.34 &    0.96  &   -2.84  & 53.47 & 0.66 & 4.56 & 10 \\
 J21402305  &     Fe I  & 5123.72 &    1.01  &   -3.06  & 42.86 & 0.63 & 4.66 & 10 \\
 J21402305  &     Fe I  & 5127.36 &    0.92  &   -3.25  & 35.50 & 0.62 & 4.62 & 10 \\
 J21402305  &     Fe I  & 5133.69 &    4.18  &    0.36  & 17.17 & 0.62 & 4.36 & 9 \\
 J21402305  &     Fe I  & 5150.84 &    0.99  &   -3.04  & 38.69 & 0.58 & 4.54 & 10 \\
 J21402305  &     Fe I  & 5151.91 &    1.01  &   -3.32  & 29.57 & 0.67 & 4.68 & 10 \\
 J21402305  &     Fe I  & 5166.28 &    0.00  &   -4.12  & 51.67 & 0.54 & 4.66 & 10 \\
 J21402305  &     Fe I  & 5171.60 &    1.49  &   -1.72  & 77.69 & 0.59 & 4.48 & 10 \\
 J21402305  &     Fe I  & 5191.45 &    3.04  &   -0.55  & 39.88 & 0.61 & 4.46 & 10 \\
 J21402305  &     Fe I  & 5192.34 &    3.00  &   -0.42  & 42.64 & 0.51 & 4.34 & 10 \\
 J21402305  &     Fe I  & 5194.94 &    1.56  &   -2.02  & 57.89 & 0.54 & 4.51 & 10 \\
 J21402305  &     Fe I  & 5198.71 &    2.22  &   -2.09  & 15.31 & 0.59 & 4.50 & 10 \\
 J21402305  &     Fe I  & 5202.34 &    2.18  &   -1.87  & 29.34 & 0.57 & 4.59 & 10 \\
 J21402305  &     Fe I  & 5215.18 &    3.27  &   -0.86  & 12.15 & 0.55 & 4.37 & 9 \\
 J21402305  &     Fe I  & 5216.27 &    1.61  &   -2.08  & 52.18 & 0.50 & 4.54 & 10 \\
 J21402305  &     Fe I  & 5225.53 &    0.11  &   -4.76  & 17.69 & 0.59 & 4.77 & 10 \\
 J21402305  &     Fe I  & 5232.94 &    2.94  &   -0.06  & 69.03 & 0.52 & 4.35 & 10 \\
 J21402305  &     Fe I  & 5263.31 &    3.27  &   -0.87  & 14.20 & 0.57 & 4.45 & 9 \\
 J21402305  &     Fe I  & 5266.56 &    3.00  &   -0.38  & 47.51 & 0.54 & 4.37 & 10 \\
 J21402305  &     Fe I  & 5281.79 &    3.04  &   -0.83  & 22.27 & 0.49 & 4.38 & 10 \\
 J21402305  &     Fe I  & 5283.62 &    3.24  &   -0.45  & 29.16 & 0.53 & 4.39 & 9 \\
 J21402305  &     Fe I  & 5307.36 &    1.61  &   -2.91  & 14.60 & 0.52 & 4.58 & 10 \\
 J21402305  &     Fe I  & 5324.18 &    3.21  &   -0.11  & 46.76 & 0.52 & 4.33 & 12 \\
 J21402305  &     Fe I  & 5332.90 &    1.56  &   -2.78  & 17.93 & 0.50 & 4.50 & 10 \\
 J21402305  &     Fe I  & 5339.93 &    3.27  &   -0.63  & 19.36 & 0.55 & 4.37 & 9 \\
 J21402305  &     Fe I  & 5341.02 &    1.61  &   -1.95  & 70.00 & 0.51 & 4.69 & 10 \\
 J21402305  &     Fe I  & 5367.47 &    4.42  &    0.44  & 13.97 & 0.53 & 4.44 & 10 \\
 J21402305  &     Fe I  & 5369.96 &    4.37  &    0.54  & 14.41 & 0.50 & 4.30 & 10 \\
 J21402305  &     Fe I  & 5371.49 &    0.96  &   -1.64  & 122.49 & 0.52 & 4.72 & 10 \\
 J21402305  &     Fe I  & 5383.37 &    4.31  &    0.64  & 22.25 & 0.52 & 4.36 & 10 \\
 J21402305  &     Fe I  & 5397.13 &    0.92  &   -1.98  & 110.32 & 0.44 & 4.72 & 10 \\
 J21402305  &     Fe I  & 5405.77 &    0.99  &   -1.85  & 112.39 & 0.47 & 4.72 & 10 \\
 J21402305  &     Fe I  & 5410.91 &    4.47  &    0.40  & 10.23 & 0.54 & 4.38 & 10 \\
 J21402305  &     Fe I  & 5415.20 &    4.39  &    0.64  & 20.83 & 0.58 & 4.41 & 10 \\
 J21402305  &     Fe I  & 5429.70 &    0.96  &   -1.88  & 116.68 & 0.48 & 4.81 & 10 \\
 J21402305  &     Fe I  & 5434.52 &    1.01  &   -2.13  & 99.22 & 0.47 & 4.73 & 10 \\
 J21402305  &     Fe I  & 5497.52 &    1.01  &   -2.82  & 64.94 & 0.47 & 4.75 & 10 \\
 J21402305  &     Fe I  & 5501.47 &    0.96  &   -3.05  & 52.98 & 0.51 & 4.73 & 10 \\
 J21402305  &     Fe I  & 5506.78 &    0.99  &   -2.79  & 65.58 & 0.48 & 4.71 & 10 \\
 J21402305  &     Fe I  & 5569.62 &    3.42  &   -0.52  & 18.89 & 0.44 & 4.41 & 9 \\
 J21402305  &     Fe I  & 5586.76 &    3.37  &   -0.11  & 37.94 & 0.44 & 4.35 & 9 \\
 J21402305  &     Fe I  & 6065.48 &    2.61  &   -1.41  & 22.55 & 0.37 & 4.43 & 10 \\
 J21402305  &     Fe I  & 6136.61 &    2.45  &   -1.41  & 37.07 & 0.38 & 4.54 & 10 \\
 J21402305  &     Fe I  & 6137.69 &    2.59  &   -1.35  & 28.38 & 0.38 & 4.47 & 10 \\
 J21402305  &     Fe I  & 6230.72 &    2.56  &   -1.28  & 39.33 & 0.41 & 4.57 & 10 \\
 J21402305  &     Fe I  & 6393.60 &    2.43  &   -1.58  & 32.03 & 0.35 & 4.58 & 10 \\
 J21402305  &     Fe I  & 6411.65 &    3.65  &   -0.59  & 10.98 & 0.36 & 4.43 & 9 \\
 J21402305  &     Fe I  & 6421.35 &    2.28  &   -2.01  & 22.24 & 0.39 & 4.62 & 10 \\
 J21402305  &     Fe I  & 6430.85 &    2.18  &   -1.95  & 27.70 & 0.36 & 4.57 & 10 \\
 J21402305  &     Fe I  & 6494.98 &    2.40  &   -1.24  & 49.05 & 0.37 & 4.49 & 10 \\
 J21402305  &     Fe I  & 6592.91 &    2.73  &   -1.47  & 17.88 & 0.39 & 4.48 & 10 \\
 J21402305  &     Fe I  & 6677.99 &    2.69  &   -1.42  & 24.12 & 0.33 & 4.54 & 10 \\
 J21402305  &     Fe I  & 7511.02 &    4.18  &    0.12  & 16.29 & 0.42 & 4.48 & 9 \\
 J21402305  &    Fe II  & 4178.86 &    2.58  &   -2.51  & 36.57 & 0.41 & 4.41 & 13 \\
 J21402305  &    Fe II  & 4416.82 &    2.78  &   -2.57  & 26.90 & 0.39 & 4.48 & 14 \\
 J21402305  &    Fe II  & 4491.41 &    2.86  &   -2.71  & 15.27 & 0.36 & 4.40 & 13 \\
 J21402305  &    Fe II  & 4508.28 &    2.86  &   -2.42  & 31.69 & 0.34 & 4.52 & 14 \\
 J21402305  &    Fe II  & 4515.34 &    2.84  &   -2.60  & 26.59 & 0.35 & 4.57 & 13 \\
 J21402305  &    Fe II  & 4576.34 &    2.84  &   -2.95  & 11.61 & 0.32 & 4.48 & 13 \\
 J21402305  &    Fe II  & 4583.83 &    2.81  &   -1.94  & 60.94 & 0.30 & 4.49 & 14 \\
 J21402305  &    Fe II  & 4620.52 &    2.83  &   -3.21  & 6.91 & 0.34 & 4.48 & 13 \\
 J21402305  &    Fe II  & 5197.58 &    3.23  &   -2.22  & 20.82 & 0.54 & 4.46 & 13 \\
 J21402305  &    Fe II  & 5234.63 &    3.22  &   -2.18  & 24.65 & 0.56 & 4.50 & 13 \\
 J21402305  &    Fe II  & 5276.00 &    3.20  &   -2.01  & 30.47 & 0.50 & 4.43 & 13 \\
 J21402305  &     Ni I  & 3452.89 &    0.11  &   -0.90  & 120.66 & 3.31 & 3.55 & 15 \\
 J21402305  &     Ni I  & 3472.54 &    0.11  &   -0.79  & 127.90 & 1.82 & 3.61 & 15 \\
 J21402305  &     Ni I  & 3500.85 &    0.17  &   -1.27  & 111.27 & 1.51 & 3.67 & 15 \\
 J21402305  &     Ni I  & 3597.70 &    0.21  &   -1.10  & 112.40 & 1.03 & 3.48 & 15 \\
 J21402305  &     Ni I  & 4470.48 &    3.40  &   -0.30  & 9.60 & 0.39 & 3.58 & 15 \\
 J21402305  &     Ni I  & 4604.99 &    3.48  &   -0.24  & 9.09 & 0.36 & 3.58 & 15 \\
 J21402305  &     Ni I  & 4648.65 &    3.42  &   -0.09  & 15.40 & 0.38 & 3.61 & 15 \\
 J21402305  &     Ni I  & 4714.42 &    3.38  &    0.25  & 28.52 & 0.34 & 3.56 & 15 \\
 J21402305  &     Ni I  & 4756.52 &    3.48  &   -0.27  & 8.51 & 0.31 & 3.56 & 15 \\
 J21402305  &     Ni I  & 4904.41 &    3.54  &   -0.17  & 14.78 & 0.38 & 3.80 & 1 \\
 J21402305  &     Ni I  & 4980.17 &    3.60  &    0.07  & 13.16 & 0.41 & 3.56 & 15 \\
 J21402305  &     Ni I  & 5017.58 &    3.54  &   -0.03  & 13.06 & 0.47 & 3.59 & 15 \\
 J21402305  &     Ni I  & 5080.53 &    3.65  &    0.32  & 17.76 & 0.65 & 3.52 & 15 \\
 J21402305  &     Ni I  & 5081.11 &    3.85  &    0.30  & 13.42 & 0.72 & 3.62 & 1 \\
 J21402305  &     Ni I  & 5084.08 &    3.68  &    0.03  & 11.69 & 0.69 & 3.63 & 1 \\
 J21402305  &     Ni I  & 5115.40 &    3.83  &   -0.11  & 6.25 & 0.60 & 3.64 & 1 \\
 J21402305  &     Ni I  & 5155.76 &    3.90  &   -0.09  & 7.38 & 0.68 & 3.78 & 1 \\
 J21402305  &     Ni I  & 6643.63 &    1.68  &   -2.22  & 18.32 & 0.36 & 3.72 & 15 \\
 J21402305  &     Ni I  & 6767.77 &    1.83  &   -2.14  & 14.41 & 0.41 & 3.68 & 15 \\
 J21402305  &     Zn I  & 4680.14 &    4.01  &   -0.85  & 21.67 & 1.25 & 2.78 & 16 \\
 J21402305  &     Zn I  & 4722.16 &    4.03  &   -0.37  & 38.79 & 0.34 & 2.67 & 16 \\
 J21402305  &     Zn I  & 4810.54 &    4.08  &   -0.15  & 43.68 & 0.33 & 2.59 & 16 \\
 J21402305  &    C-H I  & 4312.00 &     NaN  &     NaN  &     synth  &    synth  & 5.86 & NaN \\
 J21402305  &    C-H I  & 4323.00 &     NaN  &     NaN  &     synth  &    synth  & 5.85 & NaN \\
 J21402305  &    C-H I  & 4230.00 &     NaN  &     NaN  &     synth  &    synth  & 5.83 & NaN \\
 J21402305  &    C-H I  & 4311.00 &     NaN  &     NaN  &     synth  &    synth  & 5.83 & NaN \\
 J21402305  &    C-N I  & 3362.00 &     NaN  &     NaN  &     synth  &    synth  & 6.04 & NaN \\
 J21402305  &     Al I  & 3944.00 &    0.00  &   -0.64  &     synth  &    synth  & 2.82 & 1 \\
 J21402305  &     Si I  & 4102.94 &    1.91  &   -3.34  &     synth  &    synth  & 5.31 & 1 \\
 J21402305  &    Sc II  & 3572.53 &    0.02  &    0.27  &     synth  &    synth  & 0.62 & 18 \\
 J21402305  &    Sc II  & 3590.47 &    0.02  &   -0.55  &     synth  &    synth  & 0.29 & 18 \\
 J21402305  &    Sc II  & 3630.74 &    0.01  &    0.22  &     synth  &    synth  & 0.30 & 18 \\
 J21402305  &    Sc II  & 4246.82 &    0.32  &    0.24  &     synth  &    synth  & 0.16 & 18 \\
 J21402305  &    Sc II  & 4324.99 &    0.60  &   -0.44  &     synth  &    synth  & 0.03 & NaN \\
 J21402305  &    Sc II  & 4374.47 &    0.62  &   -0.46  &     synth  &    synth  & 0.09 & NaN \\
 J21402305  &    Sc II  & 4400.39 &    0.61  &   -0.54  &     synth  &    synth  & 0.06 & NaN \\
 J21402305  &    Sc II  & 4415.56 &    0.60  &   -0.68  &     synth  &    synth  & 0.10 & NaN \\
 J21402305  &    Sc II  & 4670.41 &    1.36  &   -0.60  &     synth  &    synth  & 0.21 & NaN \\
 J21402305  &    Sc II  & 5031.02 &    1.36  &   -0.41  &     synth  &    synth  & 0.09 & NaN \\
 J21402305  &    Sc II  & 5526.79 &    1.77  &   -0.01  &     synth  &    synth  & 0.13 & NaN \\
 J21402305  &    Sc II  & 5657.90 &    1.51  &   -0.54  &     synth  &    synth  & 0.22 & NaN \\
 J21402305  &      V I  & 4111.78 &    0.30  &    0.40  &     synth  &    synth  & 1.00 & 19 \\
 J21402305  &      V I  & 4379.23 &    0.30  &    0.58  &     synth  &    synth  & 1.01 & 19 \\
 J21402305  &     V II  & 3517.30 &    1.13  &   -0.24  &     synth  &    synth  & 0.93 & 20 \\
 J21402305  &     V II  & 3530.77 &    1.07  &   -0.53  &     synth  &    synth  & 0.98 & 20 \\
 J21402305  &     V II  & 3545.20 &    1.09  &   -0.32  &     synth  &    synth  & 1.09 & 20 \\
 J21402305  &     V II  & 3715.46 &    1.57  &   -0.22  &     synth  &    synth  & 1.10 & 20 \\
 J21402305  &     V II  & 3727.34 &    1.69  &   -0.23  &     synth  &    synth  & 1.36 & 20 \\
 J21402305  &     V II  & 3903.25 &    1.48  &   -0.91  &     synth  &    synth  & 1.29 & 20 \\
 J21402305  &     V II  & 3951.96 &    1.48  &   -0.73  &     synth  &    synth  & 1.15 & 20 \\
 J21402305  &     V II  & 3997.11 &    1.48  &   -1.20  &     synth  &    synth  & 1.23 & 20 \\
 J21402305  &     V II  & 4002.93 &    1.43  &   -1.44  &     synth  &    synth  & 1.28 & 20 \\
 J21402305  &     V II  & 4023.38 &    1.80  &   -0.61  &     synth  &    synth  & 1.21 & 20 \\
 J21402305  &     Mn I  & 4030.75 &    0.00  &   -0.50  &     synth  &    synth  & 2.51 & 21 \\
 J21402305  &     Mn I  & 4033.06 &     0.00  &    -0.65  &     synth  &    synth  & 2.38 & 21 \\
 J21402305  &     Mn I  & 4034.48 &    0.00  &   -0.84  &     synth  &    synth  & 2.31 & 21 \\
 J21402305  &     Mn I  & 4754.04 &    2.28  &   -0.08  &     synth  &    synth  & 2.32 & 21 \\
 J21402305  &     Mn I  & 4762.37 &    2.89  &    0.30  &     synth  &    synth  & 2.28 & 21 \\
 J21402305  &     Mn I  & 4823.52 &    2.32  &    0.14  &     synth  &    synth  & 2.32 & 21 \\
 J21402305  &    Mn II  & 3441.99 &    1.78  &   -0.35  &     synth  &    synth  & 2.42 & 21 \\
 J21402305  &    Mn II  & 3488.68 &    1.85  &   -0.94  &     synth  &    synth  & 2.34 & 21 \\
 J21402305  &    Mn II  & 3497.53 &    1.85  &   -1.42  &     synth  &    synth  & 2.27 & 21 \\
 J21402305  &     Co I  & 3455.24 &    0.22  &   -1.19  &     synth  &    synth  & 2.63 & 22 \\
 J21402305  &     Co I  & 3489.40 &    0.92  &    0.18  &     synth  &    synth  & 2.05 & 22 \\
 J21402305  &     Co I  & 3491.32 &    0.22  &   -1.41  &     synth  &    synth  & 2.42 & 22 \\
 J21402305  &     Co I  & 3502.28 &    0.43  &    0.11  &     synth  &    synth  & 2.28 & 22 \\
 J21402305  &     Co I  & 3513.48 &    0.10  &   -0.79  &     synth  &    synth  & 2.52 & 22 \\
 J21402305  &     Co I  & 3518.34 &    1.05  &    0.00  &     synth  &    synth  & 2.26 & 22 \\
 J21402305  &     Co I  & 3521.57 &    0.43  &    -0.74  &     synth  &    synth  & 2.35 & 22 \\
 J21402305  &     Co I  & 3529.03 &    0.17  &   -0.89  &     synth  &    synth  & 2.51 & 22 \\
 J21402305  &     Co I  & 3529.03 &    0.17  &   -0.89  &     synth  &    synth  & 2.45 & 22 \\
 J21402305  &     Co I  & 3550.59 &    0.17  &   -1.59  &     synth  &    synth  & 2.46 & 22 \\
 J21402305  &     Co I  & 3564.95 &    0.58  &   -0.96  &     synth  &    synth  & 2.35 & 22 \\
 J21402305  &     Co I  & 3842.05 &    0.92  &   -0.74  &     synth  &    synth  & 2.37 & 22 \\
 J21402305  &     Co I  & 3845.47 &    0.92  &    0.06  &     synth  &    synth  & 2.13 & 22 \\
 J21402305  &     Co I  & 3894.08 &    1.05  &    0.12  &     synth  &    synth  & 2.05 & 22 \\
 J21402305  &     Co I  & 3995.31 &    0.92  &   -0.18  &     synth  &    synth  & 2.30 & 22 \\
 J21402305  &     Co I  & 4118.77 &    1.05  &   -0.48  &     synth  &    synth  & 2.32 & 22 \\
 J21402305  &     Co I  & 4121.32 &    0.92  &   -0.33  &     synth  &    synth  & 2.35 & 22 \\
 J21402305  &     Cu I  & 5105.50 &    1.39  &   -1.50  &     synth  &    synth  & 1.22 & 33 \\
 J21402305  &     Sr I  & 4607.33 &    0.00  &    0.28  &     synth  &    synth  & 1.01 & 23 \\
 J21402305  &    Sr II  & 4077.71 &    0.00  &    0.15  &     synth  &    synth  & 1.41 & 23 \\
 J21402305  &    Sr II  & 4161.80 &    2.94  &   -0.47  &     synth  &    synth  & 1.37 & 23 \\
 J21402305  &    Sr II  & 4215.52 &    0.00  &   -0.17  &     synth  &    synth  & 1.46 & 23 \\
 J21402305  &     Y II  & 3600.73 &    0.18  &     0.34  &     synth  &    synth  & -0.08 & 24 \\
 J21402305  &     Y II  & 3611.04 &    0.13  &    0.05  &     synth  &    synth  & -0.04 & 24 \\
 J21402305  &     Y II  & 3628.70 &    0.13  &   -0.70  &     synth  &    synth  & 0.04 & 24 \\
 J21402305  &     Y II  & 3710.29 &    0.18  &    0.51  &     synth  &    synth  & 0.28 & 24 \\
 J21402305  &     Y II  & 3747.55 &    0.10  &   -0.95  &     synth  &    synth  & 0.01 & 24 \\
 J21402305  &     Y II  & 3774.33 &    0.13  &    0.29  &     synth  &    synth  & 0.03 & NaN \\
 J21402305  &     Y II  & 3832.89 &    0.18  &   -0.34  &     synth  &    synth  & -0.14 & 24 \\
 J21402305  &     Y II  & 3982.59 &    0.13  &   -0.56  &     synth  &    synth  & 0.09 & 24 \\
 J21402305  &     Y II  & 4358.72 &    0.10  &   -1.15  &     synth  &    synth  & -0.19 & 24 \\
 J21402305  &     Y II  & 4398.01 &    0.13  &   -0.75  &     synth  &    synth  & -0.17 & 24 \\
 J21402305  &     Y II  & 4854.86 &    0.99  &   -0.27  &     synth  &    synth  & -0.16 & 24 \\
 J21402305  &     Y II  & 4900.12 &    1.03  &    0.03  &     synth  &    synth  & -0.23 & 24 \\
 J21402305  &     Y II  & 4982.13 &    1.03  &   -1.32  &     synth  &    synth  & 0.05 & 24 \\
 J21402305  &     Y II  & 5087.42 &    1.08  &   -0.16  &     synth  &    synth  & -0.18 & 24 \\
 J21402305  &     Y II  & 5123.21 &     0.99  &    -0.79  &     synth  &    synth  & -0.29 & 24 \\
 J21402305  &     Y II  & 5200.41 &    0.99  &   -0.47  &     synth  &    synth  & -0.20 & 24 \\
 J21402305  &     Y II  & 5205.72 &    1.03  &     -0.28  &     synth  &    synth  & -0.14 & 24 \\
 J21402305  &    Zr II  & 3430.53 &     0.47  &     -0.16  &     synth  &    synth  & 0.37 & 25 \\
 J21402305  &    Zr II  & 3499.57 &    0.41  &   -1.06  &     synth  &    synth  & 0.65 & 25 \\
 J21402305  &    Zr II  & 3505.67 &     0.16  &     -0.39  &     synth  &    synth  & 0.60 & 25 \\
 J21402305  &    Zr II  & 3551.95 &     0.10  &    -0.36  &     synth  &    synth  & 0.68 & 25 \\
 J21402305  &    Zr II  & 3630.02 &    0.36  &   -1.11  &     synth  &    synth  & 0.57 & 25 \\
 J21402305  &    Zr II  & 3714.78 &    0.53  &   -0.96  &     synth  &    synth  & 0.52 & 25 \\
 J21402305  &    Zr II  & 3718.83 &     0.36  &     -1.76  &     synth  &    synth  & 0.55 & 25 \\
 J21402305  &    Zr II  & 3998.96 &    0.56  &   -0.52  &     synth  &    synth  & 0.56 & 25 \\
 J21402305  &    Zr II  & 4048.67 &    0.80  &    -0.53  &     synth  &    synth  & 0.41 & 25 \\
 J21402305  &    Zr II  & 4053.32 &     0.71  &    -1.06  &     synth  &    synth  & 0.53 & 25 \\
 J21402305  &    Zr II  & 4071.09 &    1.00  &   -1.66  &     synth  &    synth  & 0.61 & 25 \\
 J21402305  &    Zr II  & 4149.20 &    0.80  &   -0.04  &     synth  &    synth  & 0.34 & 25 \\
 J21402305  &    Zr II  & 4161.20 &     0.71  &     -0.59  &     synth  &    synth  & 0.41 & 25 \\
 J21402305  &    Zr II  & 4208.98 &     0.71  &     -0.51  &     synth  &    synth  & 0.40 & 25 \\
 J21402305  &    Zr II  & 4258.04 &    0.56  &   -1.20  &     synth  &    synth  & 0.63 & 25 \\
 J21402305  &    Zr II  & 4317.31 &    0.71  &   -1.45  &     synth  &    synth  & 0.66 & 25 \\
 J21402305  &    Zr II  & 4440.45 &     1.21  &     -1.04  &     synth  &    synth  & 0.34 & 25 \\
 J21402305  &    Zr II  & 4442.99 &     1.49  &     -0.42  &     synth  &    synth  & 0.49 & 25 \\
 J21402305  &    Zr II  & 4496.96 &    0.71  &   -0.89  &     synth  &    synth  & 0.62 & 25 \\
 J21402305  &    Zr II  & 4613.95 &    0.97  &   -1.54  &     synth  &    synth  & 0.57 & 25 \\
 J21402305  &    Ba II  & 4554.03 &    0.00  &    0.14  &     synth  &    synth  & -1.27 & 26 \\
 J21402305  &    Ba II  & 4934.08 &    0.00  &   -0.16  &     synth  &    synth  & -1.34 & 26 \\
 J21402305  &    Ba II  & 5853.68 &    0.60  &   -0.91  &     synth  &    synth  & -1.27 & 26 \\
 J21402305  &    Ba II  & 6141.71 &    0.70  &   -0.03  &     synth  &    synth  & -1.20 & 26 \\
 J21402305  &    Ba II  & 6496.90 &    0.60  &   -0.41  &     synth  &    synth  & -1.04 & 26 \\
 J21402305  &    La II  & 4077.34 &    0.24  &   -0.06  &     synth  &    synth  & -1.77 & 27 \\
 J21402305  &    Nd II  & 3991.74 &    0.00  &    -0.26  &     synth  &    synth  & -1.36 & 28 \\
 J21402305  &    Nd II  & 4109.45 &    0.32  &    0.35  &     synth  &    synth  & -1.55 & 28 \\
 J21402305  &    Nd II  & 4303.57 &    0.00  &    0.08  &     synth  &    synth  & -1.78 & 28 \\
 J21402305  &    Eu II  & 4129.72 &    0.00  &    0.22  &     synth  &    synth  & -2.73 & 29 \\
 J21402305  &    Eu II  & 4205.04 &    0.00  &    0.21  &     synth  &    synth  & -2.73 & 29 \\
 J21402305  &    Er II  & 3906.31 &    0.00  &    0.12  &     synth  &    synth  & -1.88 & 31 \\
 J21402305  &    Yb II  & 3694.19 &    0.00  &   -0.30  &     synth  &    synth  & -2.45 & 32 \\
 \hline
\end{tabular}%
}
\tablefoot{}
\end{table}
